Analyzing the Noise Robustness of Deep Neural Networks

Adversarial examples, generated by adding small but intentionally imperceptible perturbations to normal examples, can mislead deep neural networks (DNNs) to make incorrect predictions. Although much work has been done on both adversarial attack and defense, a fine-grained understanding of adversarial examples is still lacking. To address this issue, we present a visual analysis method to explain why adversarial examples are misclassified. The key is to compare and analyze the datapaths of both the adversarial and normal examples. A datapath is a group of critical neurons along with their connections. We formulate the datapath extraction as a subset selection problem and solve it by constructing and training a neural network. A multi-level visualization consisting of a network-level visualization of data flows, a layer-level visualization of feature maps, and a neuron-level visualization of learned features, has been designed to help investigate how datapaths of adversarial and normal examples diverge and merge in the prediction process. A quantitative evaluation and a case study were conducted to demonstrate the promise of our method to explain the misclassification of adversarial examples.

==> TVCG-Analyzing the Robustness of Deep Neural Networks/application.tex <==
%As part of our evaluation, we first performed a qualitative evaluation to demonstrate the effectiveness of the datapath extraction algorithm.
% \kelei{
% We performed a quantitative evaluation to verify the effectiveness of our constrained datapath extraction method.
% A case study, similar to the one used in our previous work, was conducted to illustrate the analysis process for misclassification of adversarial examples based on the extracted constrained datapathss.
% }


\begin{table*}[bt]
    \centering
    \begin{tabular}{c|c|cccccccccc|c}
    \toprule
    & & \multicolumn{10}{|c|}{Dataset 1} & Dataset 2 \\
    \midrule
       &  & jeep & schooner & banana & pizza & panda & goldfish & rosehip & snake & tusker & sunglass & 100 class (average) \\
    \midrule 
    \textbf{Top-1 Score} & DGR  & 0.000 & 0.038 & 0.039 & 0.059 & 0.051 & 0.006 & 0.000 & 0.025 & 0.000 & 0.029 & 0.011 \\
    & Ours & 0.017 & 0.076 & 0.058 & 0.078 & 0.061 & 0.029 & 0.045 & 0.025 & 0.021 & 0.057 & 0.042\\
    \midrule  
    \textbf{Top-3 Score} & DGR  & 0.033 & 0.114 & 0.107 & 0.176 & 0.111 & 0.041 & 0.061 & 0.101 & 0.042 & 0.095 & 0.064 \\
    & Ours & 0.083 & 0.253 & 0.165 & 0.333 & 0.222 & 0.110 & 0.091 & 0.139 & 0.104 & 0.152 & 0.123 \\
    \midrule  
    \textbf{Top-5 Score} & DGR  & 0.067 & 0.177 & 0.117 & 0.275 & 0.172 & 0.076 & 0.091 & 0.215 & 0.083 & 0.162 & 0.123 \\
    & Ours & 0.133 & 0.468 & 0.204 & 0.647 & 0.404 & 0.174 & 0.136 & 0.291 & 0.167 & 0.248 & 0.209 \\
    \bottomrule
    \end{tabular}
    \caption{The top -1, -3, -5 scores on the 10-class and the 100-class datasets using DGR~\cite{wang2018interpret} and our method for datapath extraction.} %Higher values are better, because it mean more merging patterns found by the method.}
    \label{tab:QuanExpr_0}
\end{table*}

\section{Evaluation}
\newdoc{%In this section, we
We} first quantitatively evaluated the effectiveness of the proposed constrained datapath extraction method in comparison with a previous state-of-the-art method, the DGR method~\cite{wang2018interpret}.
%As part of our evaluation, we first performed a quantitative evaluation to demonstrate the effectiveness of the datapath extraction algorithm.
We then demonstrated through a case study how AEVis helped the analysis of the root cause for misclassification of adversarial examples.
\jing{Expert \caseexpert{1}, one of the two experts \newdoc{who} participated in the evaluation of the previous version of AEVis~\cite{liu2018analyzing}, was invited again to evaluate the usefulness of the new system.}
%Then, we conduct a case study to illustrate how AEVis helps the expert \caseexpert{1} analyze the root cause of a misclassification introduced by an adversarial example. 
%% both white-box and black-box adversarial examples. 
% \subsubsection{Analyzing White-Box Adversarial Examples}
The CNN used for evaluation is a pretrained
%One of the state-of-the-art CNNs for image classification, 
\textbf{ResNet-101}~\cite{He2016_CVPR_residual}, which contains 101 layers and is 
\newdoc{%one of the
a} state-of-the-art CNN\newdoc{%s
} for image classification.
%is employed as the target model.
%It contains 101 layers. 
%We used the pre-trained model from TensorFlow~\cite{Tensorboard2017_web}.
%\jw{More specifically, a pretrained model in TensorFlow~\cite{Tensorboard2017_web} is used in the evaluation.}
%It achieves a high accuracy ($96.3\%$) on the normal examples, and a very low accuracy ($0.9\%$) on the generated adversarial examples.


\subsection{Quantitative Analysis}%  of Constrained Datapath Extraction
\label{sec:eval_dp}

\mc{
%In this part, we conducted a quantitative experiment to evaluate the effectiveness of the proposed constrained datapath extraction method.
As there is no ground-truth for datapaths, the effectiveness of the datapath extraction method is measured by the ability to detect the \jw{diverging-merging} patterns between the extracted datapaths.
\jw{Two datasets with different scales were used for this evaluation. One dataset contains all the images of 10 randomly selected classes 
\jw{(shown at the top of Table~\ref{tab:QuanExpr_0})} 
from ImageNet ILSVRC 2012~\cite{russakovsky2015imagenet}. The other contains 100 classes, with 10 randomly selected images in each class.}
%In particular, 
We used a state-of-the-art attacking method, namely, \newdoc{the} momentum iterative fast gradient sign method~\cite{NIPS_attack_code,dong2018boosting}, to generate an adversarial example for each image in the datasets.%for a widely-used deep CNN (ResNet-101~\cite{He2016_CVPR_residual}).
}
\jw{From the classification results of these adversarial images, for each \jing{class that was mistakenly classified into}, we further sampled $20$ %$M$ 
target images from the original ImageNet ILSVRC 2012 dataset.}
%Based on the generated adversarial examples $E_A$, we extracted the datapaths of the corresponding normal images $E_O$
\jw{Then for each misclassified adversarial image, we constructed $20$ %$M$ 
triplets of normal source/adversarial/normal target images and extracted datapaths for each triplet.}
%and calculate the ability of detecting diverging and merging patterns.
%In particular, 


As shown in Fig.~\ref{fig:case0_overview}, 
there is a diverging point (\pictag{L}{A}) where the datapath of the misclassified adversarial image gradually deviates from the datapath of the normal source image, and gets closer to that of the normal target image and merges with it at a point (\pictag{L}{E}), resulting in the misclassification.
Such a diverging followed by \newdoc{a} merging pattern (simplified as a \textbf{diverging-merging pattern}) is an important characteristic indicating the misclassification of adversarial images. The ability of the extracted datapaths to reflect such patterns is thus used to evaluate the effectiveness of the datapath extraction method.

\jw{To determine the occurrence of a diverging-merging pattern, we calculated the difference 
\newdoc{%of
in the} distances between 1) the datapaths of the adversarial and normal source images and 2) the datapaths of the adversarial and normal target images. The difference at layer $i$ is calculated as:}
\begin{equation}
\label{eq:case-pattern-diff}
diff(i) = ||\vecz{opt}^{adv}(i)-\vecz{opt}^{src}(i))||_2 -  ||\vecz{opt}^{adv}(i)-\vecz{opt}^{tar}(i)||_2
\end{equation}
where $\vecz{opt}^{adv}$, $\vecz{opt}^{src}$, and $\vecz{opt}^{tar}$ denote datapaths of the adversarial example, the normal source image that corresponds to the adversarial, and the normal target image, respectively. 

% Accordingly, if the number of layers ($n_f$) that the distance difference kept increasing towards the end of the model:
If the distance difference of the last $r$ layers
\newdoc{%keeps increasing
continues to increase} towards the end of the model, a diverging-merging pattern is detected. 
Thus, we \newdoc{%counted
count} the number of layers ($n_l$) that %with 
continuously increasing in the last $r$ layers:
 \begin{equation}
\label{eq:case-pattern-count}
%n_l = |\{i \in \mathbb{N}:\textit{diff}(i)>\textit{diff}(i-1), i\in [m\text{-}r\text{+}1, m]\}|
n_l=\sum_{i=m-r+1}^{m} \mathbb{I}(diff(i)>diff(i-1))
\end{equation}
where $\mathbb{I}(\cdot)$ is an indicator function. It equals \newdoc{%to
}1 if the predicate is true, and 0 otherwise. 
$m$ is the number of layers in the model, \jw{and $r$ is a number recommended by experts to set the minimum length of the diverging-merging pattern \todo{($r=8$ in our experiments)}. 
Then such a pattern is detected when $n_l=r$ and $diff(m)$ reaches the maximum.} 
%$i$ represents the $i$-th layer that sorted by depth.
%$r$ is recommended by experts to limit the minimal length of diverging-merging pattern.

%delta(i) = DisList(D(A), D(O))(i) – DisList(D(A), D(T))(i)

\jw{%To measure the ability, 
To evaluate the effectiveness of the datapath extraction method, we then defined the following score:} 
%\mc{
%For comparison, we also calculated such score for baseline DGR datapath extraction approach~\cite{wang2018interpret}.
%To fully evaluate our approach, we calculated the score on two datasets with different scales.
%%The first dataset contained all the images of 10 random selected classes in ImageNet ILSVRC 2012~\cite{russakovsky2015imagenet}.
%%The other one contains 100 classes that had 10 images per class.
%}

% \mc{Based on the generated adversarial examples $E_A$, we extracted the datapaths of the corresponding normal images $E_O$ and calculated the ability of detecting diverging patterns as: .
% For comparison, we also calculated such score for baseline DGR datapath extraction approach~\cite{wang2018interpret}.
% To fully evaluate our approach, we calculated the score on two datasets with different scales.
% The first dataset contained all the images of 10 random selected classes in ImageNet ILSVRC 2012~\cite{russakovsky2015imagenet}.
% The other one contains 100 classes that had 10 images per class.
% We can find that \todo{mei zuo wan}.
% Besides diverging patterns, we also calculated the score for detecting merging patterns. \todo{zen me suan de, wo zhen mei kan dong}
% }
% \kelei{
% One of the state-of-the-art CNNs for image claaification, ResNet101, is used to evaluate the proposed constrained datapath extraction method.
% The adversarial examples used in the experiment are generated by a white-box non-targeted attacking method , which is also used in our previous work.
% Two datasets that was sampled from the ImageNet ILSVRC 2012 dataset~\cite{russakovsky2015imagenet} were tested.
% One dataset contained all the images of 10 classes.
% The other one contains 100 classes that had 10 images per class.
% We denote \textbf{target-images} of an adversarial examples as images that were sampled from the class this adversarial example was misclassified as.
% }
% \kelei{
% Since our approach is aim to extract datapaths while maintaining the diverging and merging patterns of the extracted datapaths,
% we introduce frequency of occurrences of merging patterns in following measure.
% }

\noindent 
\kelei{
\textbf{Top-}\textbf{\emph{K}} \textbf{score}.
For each \jw{misclassified} adversarial example, we sorted the corresponding target images in descending order 
according to their datapath similarity (based on the distance defined in Eq.~(\ref{eq:dp-ext-new-3}), 1/dis) with the adversarial image.
%prioritized by their similarities with the adversarial example.
The top-\emph{K} score is calculated as the average number of diverging-merging patterns in the top-K target-images of \jw{each adversarial example.}
%adversarial examples is called Top-K score.
}
\jw{The higher the score, the better detection of the diverging-merging pattern in the extracted datapaths, and thus more effective the datapath extraction method.} 

We computed the top-$1$, top-$3$, and top-$5$ scores of our datapath extraction method. For comparison, we also computed the scores for the DGR method~\cite{wang2018interpret}.
% , the state-of-the-art method for datapath extraction from neural networks.
\kelei{
%We compared the extracted datapath with DGR method~\cite{wang2018interpret},
%which is also designed to extract datapath from a neural network.
%We generated an adversarial example for each image in two datasets,
% and sampled \emph{M} images from the  ILSVRC 2012 dataset as the corresponding target-images. 
%and sampled \emph{M} target-images from the  ILSVRC 2012 dataset. 
%In our experiments, M was 20, we compared Top-\emph{1}, Top-\emph{3} and Top-\emph{5} score of two methods.
Table~\ref{tab:QuanExpr_0} shows 
\jw{the computed scores on the $10$ randomly selected classes in the first dataset. It can be seen} 
that our method performs better than the DGR method on all the classes.
%almost all the classes except on `jeep' and `tusker'.
We further computed the scores on the 100 classes in the second dataset, and the average result shown in the last column of Table~\ref{tab:QuanExpr_0} further verified the effectiveness of our method.
}



\subsection{Case Study}
\label{sec:case}



% \shixia{Shixia to Mengchen and Kelei: introduce data and model first, and then the case study. for the case study, list 3-5 sub-titles}
\jw{We invited %one of the two experts 
\jing{expert} \caseexpert{1}, to evaluate the usefulness of AEVis.}
\jw{As \caseexpert{1} participated in the aforementioned NIPS 2017 adversarial attack competition, he was interested in using the same \textbf{DEV} dataset from the competition~\cite{NIPS2017_Challenge}. He would like to see whether AEVis could help him gain a better understanding of the misclassification of adversarial examples.} 
\jw{The \textbf{DEV} dataset contains 1000 images of different classes, } 
\jw{and for each image, we generated an adversarial image using the non-targeted attacking method developed by the winning team~\cite{NIPS_attack_code,dong2018boosting}. }



\jw{To facilitate the analysis,
%an adversarial score was calculated
\keleiReRe{we calculated an adversarial score}
for each adversarial image using the method in~\cite{pang2018towards}. A higher score means \newdoc{a} more
obvious \newdoc{%an
}adversarial example. These scores, together with the classification results, 
were presented to \caseexpert{1} for him to select suitable adversarial examples for analysis. \caseexpert{1} was interested in misclassified adversarial examples with medium scores, as 
he commented, `Less obvious examples often contain subtle changes with big influence'.} 
%
%There are two main types of adversarial attacks: white-box attack and black-box attack~\cite{Akhtar2018_threat}.
%The white-box attack means that the attacker has a full knowledge of the target model, including the parameters, architecture, training method, and even the training data.
%While the Black-box attack assumes that the attacker knows nothing about the target model.
%
%\kelei{
%Using our approach, the analysis process are similar for two types of attacks: first select normal examples as control groups for adversarial examples,
%then extract and visualize the datapaths of normal and adversarial examples, 
%next go deep into the CNN through our visualization and interactively compare the model's behaviors on different examples.
%Therefore, in this section, we only introduce a case study for analyzing white-box adversarial examples to validate the effectiveness of our proposed approach.
%With the help of current system, especially compared to our previous work~\cite{liu2018analyzing},
%experts is able to figure out more specific reasons of the misclassification of adversarial examples.
%}
%% Next, we demonstrate how AEVis helps analyzing both white-box and black-box adversarial examples. 
%
%% In both case studies, we utilized the dataset that is from the NIPS 2017 non-targeted adversarial attack and targeted adversarial attack competitions~\cite{NIPS2017_Challenge}.
%% It contains 1,000 images (299 pixel $\times$ 299 pixel)
%% We employed the white-box non-targeted attacking method developed by the winning machine learning group~\cite{NIPS_attack_code,dong2017boosting} to generate one adversarial example for each image in the dataset
%
%%\noindent \textbf{\normalsize Input images.}
%%\kelei{
%%The image dataset, which is used in our previous work~\cite{liu2018analyzing}, is from the NIPS 2017 non-targeted adversarial attack and targeted adversarial attack competitions~\cite{NIPS2017_Challenge}.
%%The adopted white-box non-targeted attacking method is developed by the winning machine learning group of the competition~\cite{NIPS_attack_code, dong2018boosting}.
%%%Because the analysis process for white-box adversarial examples is similar to ones for black-box adversarial examples,
%%a case study for analyzing white-box adversarial examples is adopted to demonstrate the effectiveness of our proposed approach.
%%}
%
%%% \subsubsection{Analyzing White-Box Adversarial Examples}
%
%%\noindent \textbf{\normalsize Model.}
%%One of the state-of-the-art CNNs for image classification, ResNet101~\cite{He2016_CVPR_residual}, is employed as the target model.
%%It contains 101 layers. 
%%We used the pre-trained model from TensorFlow~\cite{Tensorboard2017_web}.
%%It achieves a high accuracy ($96.3\%$) on the normal examples, and a very low accuracy ($0.9\%$) on the generated adversarial examples.
%
%\noindent \textbf{\normalsize Initialization.}
%To start the analysis, we calculated an adversarial score for each image~\cite{pang2018towards}.
%A high score means the image is most probably to be an adversarial example.
%The expert \caseexpert{1} then focused on the most uncertain images with medium adversarial scores.
After examining these uncertain adversarial examples, %\caseexpert{1} \jing{first} selected \jing{a panda image}  
%for further investigation (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}).
\jing{\caseexpert{1} selected two images for further investigation:
%. Here we present two examples
an image of a panda head 
\newdoc{%but
that had been} misclassified as a guenon monkey (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}), and an image of a cannon misclassified as a racket (Fig.~\ref{fig:case2-diverging}).}
%It is 
%an image of a panda head but misclassified as a guenon monkey.
%\jing{for further investigation: an image of a panda head but misclassified as a guenon monkey (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}), and an image of a cannon misclassified as a racket.}


% To understand the root cause of this misclassification, he wanted to compare its datapath with the one of the corresponding normal example (\pictag{I}{1} in Fig.~\ref{fig:teaser}).
% To improve the representativeness of the extracted datapath for the normal example (Sec.~\ref{sec:eval_dp}, Fig.~\ref{fig:dp_extract_set}), he added 10 more normal panda images as well as the corresponding adversarial examples, to the images of interest (\textbf{R1}).
% Each added adversarial example is misclassified as a guenon monkey.
% Accordingly, the expert split these images into two sets.
% The first set (adversarial group) contained 11 adversarial examples.
% The second set of images (normal group) contained 11 normal examples.
% Then he extracted and visualized the datapaths for these two sets of images.

\jing{\subsubsection{Panda image}}
\label{sec:panda}
\kelei{
To \jw{find and} understand the root cause of this misclassification, \caseexpert{1} 
\jw{selected the adversarial panda image (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}), the normal panda image (\pictag{I}{1} in Fig.~\ref{fig:teaser-overview}), and $10$ normal guenon monkey images (\pictag{I}{3} in Fig.~\ref{fig:teaser-overview}) in the AEVis system.} 
%wanted to compare its datapath with the one of the corresponding normal panda example and the ones of normal guenon monkey images
%He split these images into three groups as the input of our system: panda group, adversarial group and monkey group.
%The adversarial group contained the selected adversarial panda image (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}).
%The panda group contained the normal panda image (\pictag{I}{1} in Fig.~\ref{fig:teaser-overview}).
%The monkey group contained 10 normal monkey images (\pictag{I}{3} in Fig.~\ref{fig:teaser-overview}).
% The datapaths of normal and adversarial panda images and a representative monkey image that have the datapath most similar to adversarial example, were then automatically extracted for further analysis.
The datapaths of normal and adversarial panda images and a representative monkey image were then automatically extracted for further analysis.
\mcrev{In particular, the representative monkey image was selected from $10$ randomly sampled monkey images, \newdoc{among which it had} the highest datapath similarity with the adversarial panda image (Eq.~\ref{eq:dp-ext-new-3}).
%we selected the monkey image as the one with the highest datapath similarity (Eq.~\ref{eq:dp-ext-new-3}) in $10$ randomly-sampled monkey images.
}
%that have the datapath most similar to adversarial example
}

% \begin{figure}[htbp]
%   \centering
%   \begin{overpic}[width = 0.98\linewidth]{fig/case-dataflow.pdf} %fig/eval_datapath_overview.pdf}
%   \small
%   %\put(-3, 40){(a)}
%   \put(5,-3){$\textsf{L}_\textsf{A}$}
%   \put(27,-3){$\textsf{L}_\textsf{B}$}
%   \put(50,-3){$\textsf{L}_\textsf{C}$}
%   \put(71,-3){$\textsf{L}_\textsf{D}$}
%   \put(92,-3){$\textsf{L}_\textsf{E}$}
%   \end{overpic}
%   \vspace{3mm}
  
%   %\begin{overpic}[width=0.8\linewidth]{fig/case-dataflow-simple.pdf} %fig/eval_datapath_overview.pdf}
%   %\put(-10, 20){(b)}
%   %\put(49,35.5){Diverging}
%   %\put(80,35.5){Merging}
%   %\put(51,-1){$\mathrm{L_A}$}
%   %\put(63,-1){$\mathrm{L_B}$}
%   %\put(81,-1){$\mathrm{L_C}$}
%   %\put(100,-1){$\mathrm{L_D}$}
%   %\end{overpic}
%   %\vspace{1mm}
%   \caption{\jw{Layers} %Area 
%   of interest in datapath overview that reflect a diverging and merging pattern.
%   Different curves represent different input \jw{images}  %image groups 
%   (\pictag{I}{1}, \pictag{I}{2}, \pictag{I}{3} in Fig.~\ref{fig:teaser-overview}(a)).}
% %     \vspace{-2mm}
%   %(c) critical neurons found by our back-propagation based approach.}\looseness=-1
%   \label{fig:case0_overview}
% \end{figure}

 
\begin{figure}[bp]
  \centering
  \begin{overpic}[width=0.99\linewidth]{fig/f_d_e.pdf}
  \small
  \end{overpic}
  \caption{
  \kelei{Activation of feature maps in (a) \pictag{L}{A}, (b) \pictag{L}{D} and (c) \pictag{L}{E}.}
  %Activation of feature maps in \pictag{L}{D} (left) and \pictag{L}{E} (right) on the normal and adversarial panda images.
  }
  \label{fig:f_d_e}
\end{figure}

\begin{figure*}[tb]
  \centering
  \vspace{2mm}
  \scriptsize
  \begin{overpic}[width=0.98\linewidth]{fig/case-merging_overview.pdf}
  \put(42.5, 55.5){\textsf{Direction for merging analysis}}
  \put(2.5, 18){\begin{sideways}\textsf{Analysis for a single feature map}\end{sideways}}
  \put(7, 37){\begin{sideways}\textsf{(i) Layer-level}\end{sideways}}
  \put(9, 37){\begin{sideways}\hspace{2mm}\textsf{visualization}\end{sideways}}
  \put(7, 20.5){\begin{sideways}\textsf{(ii) Learned}\end{sideways}}
  \put(9, 20.5){\begin{sideways}\hspace{3mm}\textsf{features}\end{sideways}}
  \put(7, 7){\begin{sideways}\textsf{(iii) Activation}\end{sideways}}
  \put(9, 7){\begin{sideways}\hspace{5mm}\textsf{maps}\end{sideways}}
   \put(95.8, 32.5){$\textsf{F}_\textsf{E}$}
   \put(66.2, 48){$\textsf{F}_\textsf{C2}$}
   \put(37, 45.5){$\textsf{F}_\textsf{B}$}
    \put(72, 30.5){$\textsf{L}_\textsf{E}$}
   \put(42.2, 30.5){$\textsf{L}_\textsf{C}$}
   \put(12.5, 30.5){$\textsf{L}_\textsf{B}$}
   \put(99.3, 18){\textsf{A}}
  \put(11.5, 3){\textsf{(a)}}
  \put(41.2, 3){\textsf{(b)}}
  \put(71, 3){\textsf{(c)}}
  \put(42, -0.5){\textsf{Direction of dataflow in the model}}
  \end{overpic}
  \vspace{2mm}
\caption{
\kelei{\caseexpert{1}'s analysis process from the deep layer \pictag{L}{E} to the shallow layer \pictag{L}{B} 
\newdoc{%for finding
in order to find} the major cause of merging.}}
  \label{fig:case-merging-overview}
\end{figure*}

\noindent \textbf{\normalsize Overview.}
\kelei{
\jw{The system first displayed the datapaths at the network-level (Fig.~\ref{fig:teaser-overview} (b)).
%(Fig.~\ref{fig:case0_overview}). 
The distances among the three datapaths disclose the diverging-merging patterns through the layers.}
%The relations among datapaths of three groups were visualized as the distance among curves in datapath overview (Fig.~\ref{fig:case0_overview}).
%
%Three lines for groups were near each other at the beginning of the neural network, which means datapaths of three groups were almost similar at these layers.
%Because the neurons in these layers detected basic patterns that appeared in all three images.
%As the expert expected, the datapath of monkey image first left away with the increasing depth of layers.
%And then at layer \caselayer{A}, the datapath of adversarial panda image started to leave from the one of normal panda image and gradually got close to the one of monkey image.
\jw{Following the dataflow in the overview, \caseexpert{1}} found that the datapath of the adversarial panda image 
%started to leave 
\jw{began to deviate 
from the datapath of the normal panda image at layer \caselayer{A} (Fig.~\ref{fig:case0_overview}), gradually got closer to the datapath of the monkey image, and finally merged into it at \caselayer{E} (Fig.~\ref{fig:case0_overview}).} 
%and finally at \caselayer{D}, the datapath of adversarial group merged into the datapath of monkey group.
%Based on this finding, he located 
\jw{From \caselayer{A} to \caselayer{E} are} the layers where the predictive behaviors of neurons were misled by the adversarial noise. 
To \jw{better} understand the %mechanisms 
\jw{working mechanism} 
of adversarial noise, 
% he would like to analyze the misclassification from two aspects: 
he then analyzed the misclassification from two aspects: 
the \textbf{diverging process} of the adversarial image from the normal source image (panda), and 
%(panda group and adversarial group) and 
the \textbf{merging process} of the adversarial image into the normal target images (monkey).
}



%\noindent \textbf{\normalsize Analysis for Diverging.}
\noindent \textbf{\normalsize Diverging analysis}.
To analyze which feature map\mc{s} \jw{in the datapath of the adversarial example} \mc{were} critical for the divergence,  \caseexpert{1} first expanded \jw{layer \caselayer{C} where the divergence became noticeably large.}
%the diverging point (layer \caselayer{C} in Fig.~\ref{fig:case0_overview}).
\kelei{
The encoded value of each feature map 
% in the feature map overview 
was set as the activation difference between \jw{the normal \mc{source}} %panda group 
and \jw{adversarial images.}
%adversarial group (activation difference = activations of the panda image - activations of the adversarial image).
%\doc{The large activation difference indicated that the corresponding feature map detected its learned features in the normal panda image but did not detect such a feature in the adversarial example.}
\jw{A large difference indicates that the feature map
\newdoc{%detects
has detected} its learned features in the normal source image but not in the adversarial example.}
%Because the feature map \casefm{B} in Fig.? showed the largest activation difference, he first checked its details.
\jw{With this understanding, \caseexpert{1}} directly checked the feature map \jw{\pictag{F}{C1}}, which had the largest activation difference \jw{in \pictag{L}{C}}. 
\doc{
By examining the learned features (Fig.~\ref{fig:teaser-overview}A) of this feature map, he discovered that the neurons in this feature map were trained to detect a black circle pattern that resembled an ear or an eye of a panda (Fig.~\ref{fig:teaser-overview}B and C).
\jw{Such a pattern is \mc{one of} the unique characteristics of a panda and is thus critical for its classification.}
\jw{Then looking at the activation maps (Fig.~\ref{fig:teaser-overview}C), \caseexpert{1} noticed that the neurons covering the ear area were correctly activated for the normal panda image, indicating a successful detection of this critical pattern. However, the same neurons were not activated for the adversarial example. \caseexpert{1} considered this was an important reason for the misclassification.}
%Such a feature is critical for identifying a panda, which did not appear in the adversarial example. 
}
}


\jw{To analyze the root cause for this failed detection,} 
\kelei{
%\jw{Interested in these neurons covering the ear area,} 
%Since the feature was identified by the neurons at the top right corner of the feature map 
%the expert \caseexpert{1} 
\caseexpert{1} selected \newdoc{%these
the} neurons covering the ear area to form an \todo{area of interest} (Fig.~\ref{fig:teaser-overview}D) for
\jw{a closer examination.} 
%of their working mechanisms.} 
%avoid the influence of neurons in other regions in subsequent analysis.
%\jw{The values recorded in the feature map overview were then updated with calculations carried out in this focused area only.}
%When the focused area was set, the statistical value of each feature map in feature map overview was only calculated with the neurons in this region. \todo{how to introduce this clearly?}
%\jw{Without the influence from other neurons, the activation difference in this feature map at \pictag{L}{C} became more prominent.} 
%\jw{\caseexpert{1} suspected this big difference was gradually developed through previous layers.}
%Before he expanded the layer that was at the beginning of the diverging process (\caselayer{A} in Fig.~\ref{fig:teaser-overview} (b)),
%\jw{To verify it,} 
He suspected the failed detection was influenced by the feature maps from previous layers.
% He thus set in the system the value recorded in each feature map as `contribution' to the selected one, i.e. the focused area in \casefm{C1}, 
He then set the value encoded in each feature map as the `contribution' to the selected one, i.e. the \todo{area of interest} in \casefm{C1}, 
\jw{and expanded \pictag{L}{A}, the layer at the beginning of the diverging process.} 
\jw{In the treemap-based visualization at \pictag{L}{A}, \caseexpert{1} found that feature map \casefm{A} (Fig.~\ref{fig:teaser-overview} (b)) which had the largest contribution to the activation difference in \casefm{C1}.} 
%Then in layer \caselayer{A}, he was able to find feature maps of interest that detected the components of the feature identified by feature map \casefm{B}. 
%A feature map (\casefm{A} in Fig.~\ref{fig:teaser-overview} (b)) in the datapath of panda group was found that had the largest contribution.
By examining its learned features (Fig.~\ref{fig:teaser-overview}E), \caseexpert{1} confirmed that 
\jw{it was trained for low-level detection of black-white boundaries.}
%it was trained to detect a dark color circle on top of a light color area (Fig.~\ref{fig:teaser-overview}E).
\jw{The activation maps (Fig.~\ref{fig:f_d_e} (a)) showed that this feature was detected in the normal panda image but not in the adversarial example. \caseexpert{1} speculated that this failed detection led to the failed detection of the panda's ear in \casefm{C1}, and finally led to the failed classification of the adversarial example as a panda.}
%Because this feature at the top right corner of the adversarial panda image was not detected,
%neurons in \casefm{B} failed to detect a ear of a panda at the same area, and finally failed to classify the adversarial example as a panda image.\todo{is this inference too weak?}
}



\jw{To confirm his speculation, \caseexpert{1} repeated the analysis on \pictag{L}{D} and \pictag{L}{E}. 
\newdoc{%He
In these two layers, he} selected \newdoc{%in the two layers
}several feature maps with a big activation difference between the normal and adversarial images.
From the activation maps, he found \newdoc{%some
}more significant
\newdoc{%missing
misses in the} detection of critical patterns in the adversarial example (Fig.~\ref{fig:f_d_e} (b), and (c)). Selecting the area of interest and tracing the contribution back to \pictag{L}{A}, \caseexpert{1} identified the same feature map \pictag{F}{A} as the biggest contributor to the failed detection in \pictag{L}{D} and \pictag{L}{E}.
At this point, \caseexpert{1} was convinced that the missing detection of the \newdoc{%black white
black-white} boundary in \pictag{F}{A}
\newdoc{%is
was} the root cause for the failed detection of critical patterns in higher levels
\newdoc{%which
that} finally led to the failed classification of the adversarial example as a panda.}




%\noindent \textbf{\normalsize Analysis for Merging.}
\noindent \textbf{\normalsize Merging analysis}.
\jw{After analyzing the 
\newdoc{%cause for
reason why} the adversarial example 
\newdoc{%not being
was not} classified as a panda, \caseexpert{1} turned his attention to why it was classified as a monkey.}
%The above analysis explains why the CNN failed to classify the adversarial example as a panda, but cannot explain why the image is classified as a monkey.
\jw{He suspected that the same region that led to the failed \newdoc{classification of panda} actually contributed to 
\newdoc{%the
its} classification as a monkey.}
%Inspired by the above analysis, the expert \caseexpert{1} 
\jw{Therefore, he \newdoc{%thus kept the 
retained the same}} \todo{area of interest} %to further verify whether the adversarial noise on this area led to the identification of monkey.
%Then he 
and expanded 
\newdoc{%the
}layer \caselayer{E} (Fig.~\ref{fig:case0_overview}), the merging point for the datapaths of the adversarial and the monkey images.
%From the intersection of datapaths for adversarial and monkey group,
%he wanted 
To find the feature maps that 
\newdoc{%have
had} the main contribution to the misclassification, 
%Therefore, 
he set the encoded value of each feature map as the `contribution' to the prediction of the adversarial panda image 
\jw{and identified \newdoc{the} feature map (\casefm{E} in Fig.~\ref{fig:case-merging-overview} (c)) with the largest contribution.}
%As he expected, a feature map (\casefm{E} in Fig.~\ref{fig:case-merging-overview} (c)) with the largest contribution were found.
After examining its learned features (Fig.~\ref{fig:case-merging-overview} (c)(ii)),
\caseexpert{1} discovered that it was trained to detect monkeys in various situations.
\jw{Comparing the activation maps of the adversarial example and normal monkey image (Fig.~\ref{fig:case-merging-overview} (c)(iii)), he found that the monkey face was activated in the monkey image as expected.
However, it 
\newdoc{%is
was} hard to explain the activation at the top part of the adversarial example. Intuitively, there were no indications of \newdoc{a} monkey in that part.}
%After comparing the activation heatmaps of normal and adversarial panda image (Fig.~\ref{fig:case-merging-overview} (c)(iii)),
%he found that the top right corner of the adversarial example was identified as a guenon monkey, which agreed with his previous conjecture.
Thus, \caseexpert{1} decided to trace back to the lower levels to seek more clues.



%As \caseexpert{1} found that the region of this feature was not exactly the same as the focused area,
%he adjusted the focused area carefully for further analysis.
%Similarly set the value of each feature map as contribution to feature map \casefm{E},
\jw{Guided by the larger activation on the activation map of the adversarial example, \caseexpert{1} first adjusted the \todo{area of interest} to include the most activated neurons at this layer (Fig.~\ref{fig:teaser-overview}D), and then analyzed the contributions to \pictag{F}{E} from the feature maps in previous layers.} 
%Similarly using the contribution analysis on feature map \casefm{E},
%he then looked back on \caselayer{C} (Fig.~\ref{fig:case0_overview}) to find feature maps that were responsible for the feature.
\jw{In layer \caselayer{C}, he found feature map \pictag{F}{C2} (Fig.~\ref{fig:case-merging-overview} (b)), which 
\newdoc{%has
had} the highest contribution to \pictag{F}{E}.} 
%There is a feature map (\casefm{D} in Fig.~\ref{fig:case-merging-overview} (b)) with the largest contribution in the intersection of datapaths for adversarial and monkey group.
\jw{\newdoc{%At
After} a closer look, the neurons in \pictag{F}{C2} seemed to detect the face of a monkey}  (Fig.~\ref{fig:case-merging-overview} (b)(ii)). 
%showed that the neurons inside were mainly used to detect the face of a monkey.
\jw{Activation on the monkey image was correctly located in the middle of the monkey face, but in the adversarial panda image, \newdoc{it} was again located on the top right part as was \newdoc{the case} in \pictag{F}{E} (Fig.~\ref{fig:case-merging-overview}\keleiRe{
%A
(c)}). }
\jw{`Are there patterns of a monkey face?' With this question \newdoc{in mind}, \caseexpert{1} carefully compared the adversarial example and the monkey image (Fig.~\ref{fig:case-merging-overview} (b)(iii)). He found that for the adversarial example, in the activated region, the dark strip with two lighter patches 
\newdoc{%aside
on either side} did resemble \newdoc{the look of} a monkey's nose with lighter cheeks 
\newdoc{%aside
next to it}.}
%Therefore, \caseexpert{1} confirmed that a monkey face was identified at the top right corner of the adversarial panda image. 
%\doc{
%This behavior of the CNN was unexpected because there was no monkey face in the adversarial panda image at the first glance.
%By carefully comparing the adversarial example and the monkey example (Fig.~\ref{fig:case-merging-overview} (b)(iii)), he found that there was a dark strip with a bright strip on each side at the top right corner of the adversarial panda image, which looks similar with the face of a monkey. 
%}

%\doc{
%However, this region in the normal panda image was not identified as a monkey face.}
\jw{However, the same pattern was \newdoc{%presented
present} in the normal panda image, but it was not detected by the neurons in \pictag{F}{C2}.} 
\jw{\caseexpert{1} thus wanted to investigate \keleiReRe{the} more fundamental cause 
\newdoc{%to
for} the detection.} 
%Therefore, to investigate the more basic effect of the adversarial noise, \caseexpert{1} 
\jw{Again, he adjusted the \todo{area of interest} according to the activation map and expanded} 
%He expanded 
the previous layer \caselayer{B} (Fig.~\ref{fig:case0_overview}). 
\jw{He identified \newdoc{that} feature map \pictag{F}{B} (Fig.~\ref{fig:case-merging-overview} (a)) \newdoc{%that
}was in the datapath intersection for both the adversarial and monkey images and had the largest contribution to \casefm{C2}.} 
%With the help of contribution analysis, a feature map (\casefm{C} in Fig.~\ref{fig:case-merging-overview} (a)) with the largest contribution to feature map \casefm{D} was found in the intersection of datapaths for adversarial and monkey group. 
%he found a feature map (\casefm{C} in Fig.~\ref{fig:case-merging-overview} (a)) in the intersection of datapaths for adversarial and monkey group, which had the largest contribution to feature map \casefm{D}.
Examining the learned features of this feature map (Fig.~\ref{fig:case-merging-overview} (a)(ii)),
\caseexpert{1} found that the neurons inside were trained to identify the eyes of different animals. 
 %, including monkey’s eyes.
Further inspecting the activation of the three images, he found that \jw{a small region with the appearance of an eye was detected} at the top right corner of the adversarial panda image. 
%(Fig.~\ref{fig:case-merging-overview} (a)(iii)).
(Fig.~\ref{fig:case-end}).
\jw{And compared with the normal image, this seemed attributed to the added adversarial noise.} 
\jw{In addition, the position of the `eye' combined with the position of the `nose' detected in \pictag{F}{E} resembled the layout of a real monkey face.} 
%He further discovered that the feature (eye of monkey) was located exactly at the position of an eye on a monkey face if he assumed the focused area as a monkey’s face.
%Based on this finding, 
\jw{\newdoc{%To
At} this point, \caseexpert{1}} 
figured out the effect of the adversarial noise.
The top right corner of the adversarial panda image had some similarities with a monkey's face.
In particular, the imperceptible adversarial noise misled the model to detect a monkey's eye first, 
\jw{then the subtle changes in image layout misled the model to detect a monkey's face. It was like a domino effect and finally led to the misclassification of the adversarial example as a monkey.}
%was identified by the model.
%\doc{
%It is a recognizable attribute for a guenon monkey, which made the CNN mispredict the adversarial example as a monkey.}
%}


\begin{figure}[thbp]
  \centering
  \begin{overpic}[width=0.8\linewidth]{fig/case-end.pdf}
  \small
  \end{overpic}
  \caption{A small region with the appearance of an eye was detected at the top right corner of the adversarial panda image.}
  \label{fig:case-end}
\end{figure}


\noindent \textbf{\normalsize Summary.} From the above analysis, \caseexpert{1} summarized two effects of the adversarial noise. 
%were summarized by the expert \caseexpert{1}.
The first one was that 
%the component of the panda’s ear became confused, which led to the absence of the panda’s ear in the adversarial panda image.
\jw{the outline of the panda's ear was affected by the noise, which led to the failed detection of the ear and} 
resulted in the large decrease of the predicted probability of the panda class.
The second one is that the adversarial noise misled the model to detect a monkey's eye in the same region, which further led to the detection of a monkey's face.
Then the probability of monkey class largely increased and resulted in the final misclassification.

\begin{figure}[htbp]

  \centering
  \begin{overpic}[width=0.98\linewidth]{fig/case2-fig1.pdf}
  \small
  \end{overpic}
  \caption{
  \kelei{Diverging analysis for an adversarial cannon image.}
  %Activation of feature maps in \pictag{L}{D} (left) and \pictag{L}{E} (right) on the normal and adversarial panda images.
  }
  \label{fig:case2-diverging}
\end{figure}


\jing{\subsubsection{Cannon image}}
\label{sec:cannon}
\jing{\caseexpert{1} carried out a similar examination 
\newdoc{on} the adversarial cannon image. Examining the datapaths of the normal and adversarial cannon images and a representative racket image (Fig.~\ref{fig:case2-diverging}), \caseexpert{1} first identified the diverging and merging points (\caselayer{B} and \caselayer{C} in Fig.~\ref{fig:case2-diverging}).
To analyze the root cause for divergence, \caseexpert{1} followed the same process as above. He first discovered the activation difference between the normal and adversarial images on \newdoc{%the
}feature map \casefm{B1} that was trained to detect the wheel of a cannon (Fig.~\ref{fig:case2-diverging}). He then traced the failed detection to \newdoc{%the
}feature map \casefm{A} in \caselayer{A}, where the wheel shafts were not detected in the adversarial example (Fig.~\ref{fig:case2-diverging}). \caseexpert{1} speculated the added noise blurred the edges of the shafts which resulted in the failed detection, and further led to the failed detection of the wheel, and finally the misclassification.}

\begin{figure}[htbp]
  \centering
  \begin{overpic}[width=0.95\linewidth]{fig/case2-fig2.pdf}
  \small
  \end{overpic}
  \caption{
  \kelei{Merging analysis for adversarial cannon image.}
  %Activation of feature maps in \pictag{L}{D} (left) and \pictag{L}{E} (right) on the normal and adversarial panda images.
  }
  \label{fig:case2-merging}
\end{figure}


%\jing{\caseexpert{1} then expanded \caselayer{B} and noticed the feature map \casefm{B1} which has the largest activation difference between the normal and adversarial images (Fig.3). Examining the learned features of \casefm{B1}, he discovered that the neurons in this feature map were trained to detect wheels of a cannon. Such a pattern is one of the most unique characteristics of a cannon and is thus critical for its classification. Then looking at the activation maps, \caseexpert{1} noticed that the neurons covering the wheel area (Fig. 3B) were correctly activated for the normal cannon image, indicating a successful detection of this critical pattern. However, the same neurons were not activated for the adversarial example (Fig. 3C). \caseexpert{1} considered this was an important reason for the misclassification.
%Further analyzing the contribution to the activation in this area, \caseexpert{1} expanded \caselayer{A}, the layer at the beginning of the diverging process, and noticed the feature map \casefm{A} that has the largest contribution to the activation difference in \casefm{B1} (Fig. 4). The learned feature shows that it is trained for low-level detection of wheel shafts. The activation maps (Fig. 4B and C) showed that this feature was detected in the normal cannon image but not in the adversarial example. \caseexpert{1} speculated that this failed detection led to the failed detection of the cannon’s wheel in \casefm{B1}, and finally led to the failed classification of the adversarial example as a cannon.}

\jing{To understand why the adversarial example was misclassified as a racket, \caseexpert{1} turned his attention to the merging point \caselayer{C}, and identified the feature map \casefm{C} which had the largest contribution to the misclassification (Fig.~\ref{fig:case2-merging}). Comparing the activation maps (Fig.~\ref{fig:case2-merging}\caselayer{C}), he found two regions (Fig.~\ref{fig:case2-merging}A and B) that were wrongly activated in the adversarial cannon image. Selecting each region and tracing back to layer \caselayer{B}, \caseexpert{1} noticed the feature maps that contributed the most to each of the regions were trained to detect `net' and `racket throat' respectively (Fig.~\ref{fig:case2-merging}C and D).
There are similarities between the streaks on the ground and a racket \mcrev{net}, % head
and between the gun mount and a racket throat. However, the added noise in the adversarial image 
\newdoc{%givesf
creates a} stronger activation in the two feature maps (Fig.~\ref{fig:case2-merging}\caselayer{B}). \caseexpert{1} thus speculated that the stronger activation together with the failed detection of the wheel misled the model to detect the \mcrev{net} and the throat of a racket in adjacent regions, which finally led to the misclassification of the adversarial image. %head
}



% \kelei{
% The expert firstly expanded the $\mathrm{L}_C$  (Fig.~\ref{fig:case0_overview}) to examine the most class-related information of examples.
% After checking the importance of the adversarial example on "monkey's datapath" (Fig.~\ref{fig:case0_examineUnit3} (b)),
% the expert found that neurons in a critical feature map $\mathrm{F}_C$ (Fig.~\ref{fig:case0_examineUnit3} (c)) were trained for detecting the face of a monkey (Fig.~\ref{fig:case0_examineUnit3} (e)),
% which had the largest activation on the top right cornor of the adversarial example (Fig.~\ref{fig:case0_examineUnit3} (d)).
% This behavior of the model was unexpected because there was no monkey face in the adversarial example at first glance.
% }

% \begin{figure}[!t]
%   \centering
% %   \vspace{-4mm}
%   \begin{overpic}[width=0.9 \linewidth]{fig/case0_examineUnit3.PNG}
%   \put(-5,80){(a)}
%   \put(-5,50){(b)}
%   \put(90,4){(c)}
%   \put(62,97){(d)}
%   \put(85,97){(e)}
%   \put(48, 40){$\mathrm{F}_C$}
%   \end{overpic}
%   \begin{overpic}[width=0.9\linewidth]{fig/case0_examineUnit1.PNG}
%   \put(-5,65){(f)}
%   \put(3,17){(h)}
%   \put(90,3){(g)}
%   \put(50, 57){$\mathrm{F}_B$}
%   \end{overpic}
%   \vspace{-2mm}
%   \caption{Examination of interested feature maps. The CNN erroneously detects a monkey's face: (a) input images; (b) and (f) are overviews of feature maps; (c) and (g) are details of specific feature maps; (d) activated region on adversarial example; (e) learned feature; (h) learned feature and activated region on adversarial example.}
%   %(c) critical neurons found by our back-propagation based approach.}\looseness=-1
%   \label{fig:case0_examineUnit3}
%   \vspace{-4mm}
% \end{figure}

% \kelei{
% Therefore, to analyze how the model misclassify the head of panda as a monkey face,
% the expert directly inspect the merging point $\mathrm{L}_B$, since the largely increased similarity meant big change on the mechanisms of critical neurons.
% He set the color encoding of each feature map in $\mathrm{L}_B$ as the contribution to the interested feature map $\mathrm{F}_C$.
% After examining some feature maps (Fig.~\ref{fig:case0_examineUnit3} (f)) with high contribution to feature map $\mathrm{F}_C$,
% the expert found a feature map $\mathrm{F}_B$ (Fig.~\ref{fig:case0_examineUnit3}) with the same No. (603 in Fig.~\ref{fig:case0_examineUnit3} (g)).
% He compared its learned feature and activated region (Fig.~\ref{fig:case0_examineUnit3} (h)) with feature map $\mathrm{F}_C$ and found very similar mechanisms of two feature maps.
% The expert thought it is caused mainly by the shortcuts that directly connect two feature maps,
% which is an important structure in ResNet101.
% To further analyze why the forehead of the panda is recognized as the face of a monkey, 
% he expanded the previous layer $\mathrm{L}_A$ (Fig.~\ref{fig:case0_overview}) and similarly set the color encoding of each feature map as the contribution to feature map $\mathrm{F}_B$.
% He examined the feature map with the largest importance (Fig.~\ref{fig:case0_examineUnit23}).
% The learned feature and the activated region on monkey example indicated that this feature map might be trained to detect left faces of monkeys.
% }

% \kelei{
% To confirm the mechanism of this feature map, the expert then collected activations on it from 1300 monkey images in the ILSVRC 2012 dataset,
% and found that 65\% of 200 most activated images had the largest activation at the positions of left faces,
% which indicated the feature map is mostly activated by left faces of monkeys.
% More specifically, he thought the recognized pattern was an area that had a dividing line from left down to right up with dark hair on one side and light hair on the other side.
% Further more, the expert inspected the other feature maps in layer $\mathrm{L}_A$ and finally found a symmetrical one that was trained to detect right faces of monkeys,
% which did not appear in the datapath of the adversarial example.
% As a result, the expert confirmed that the forehead of the panda in the adversarial example ($\mathrm{I}_B$ in Fig.~\ref{fig:teaser-overview}) was recognized as the left face of a monkey in layer $\mathrm{L}_A$,
% which led to the final misclassification.
% }

% \begin{figure}[!t]
%   \centering
% %   \vspace{-4mm}
%   \begin{overpic}[width=0.9 \linewidth]{fig/case0_examineUnit23.PNG}
%   \end{overpic}
%   \caption{The feature map that trained to detect left faces of monkeys.}
%   \label{fig:case0_examineUnit23}
%   \vspace{-4mm}
% \end{figure}

% \kelei{
% Finally, with the help of the new approach, the expert figured out a more specific reason of the misclassification compared with our previous work.
% }

% The datapath overview is shown in Fig.~\ref{fig:case0_overview}.
% The dot plots encoded the activation similarity between these two datapaths.
% The expert found that at the bottom layer of the network (Fig.~\ref{fig:case0_overview}\pictag{L}{A}), the activation similarity is almost 1.0 (the dot is on the right).
% This similarity remained to be 1.0  until layer \pictag{L}{B} in Fig.~\ref{fig:case0_overview}.
% After layer \pictag{L}{B}, layer \pictag{L}{C} appears as a ``diverging point'', where the activation similarity largely decreased (\textbf{R4}).
% In the following layers, the activation similarity continued decreasing to 0 (\pictag{L}{D}, \pictag{L}{E}, $L_F$), which resulted in the misclassification. 


% To analyze which feature map is critical for the divergence, the expert expanded the diverging point \pictag{L}{C} (Fig.~\ref{fig:teaser}).
% In addition, he set the color coding of each feature map as the activation difference between two sets of examples (activation difference $=$ activations of normal images $-$ activations of adversarial examples).
% A large activation difference indicates that the corresponding feature map detects its learned feature in the normal images but did not detect such a feature in the adversarial examples. 
% Because the feature map \pictag{F}{C1} in Fig.~\ref{fig:teaser} shows the largest activation difference, he then checked its neurons.
% By examining the learned feature of the neurons (Fig.~\ref{fig:teaser}A), he discovered that the neurons learned to detect a black patch that resembles a panda's ear (Fig.~\ref{fig:teaser}B and C).
% Such a feature is critical for detecting a panda's face, which does not appear in the adversarial example.
% To further investigate the influence of this feature map, the expert continued to expand the next layer (layer \pictag{L}{D}).
% He found that there was a large activation difference on the feature map for detecting a panda's face (\pictag{F}{D} in Fig.~\ref{fig:teaser}).
% This indicates that the corresponding feature map, \pictag{F}{D}, fails to detect a panda's face, which is a direct influence of the large difference on \pictag{F}{C1}.
% By the same analysis, the expert found that in the layer that detected the highest-level features (\pictag{L}{E}), there was also a large activation difference on the feature map for detecting a panda's face. 
% As the target CNN cannot detect a panda's face in highest-level features, the CNN failed to classify the adversarial example as a panda image.


% The above analysis explains why the CNN failed to classify the adversarial example as a panda, but cannot explain why the adversarial example is classified as a monkey.
% Thus, the expert compared the adversarial example with the corresponding example and a set of normal monkey images (Fig.~\ref{fig:case0_monkey} (a)).
% Triggered by the above analysis, the expert directly expanded layer \pictag{L}{C} (diverging point), and examined its feature maps (Fig.~\ref{fig:case0_monkey} (b)).
% After checking the activations of the adversarial example on the ``monkey's datapath'', the expert found that the activations were the largest on the feature map for detecting the face of a monkey (Fig.~\ref{fig:case0_monkey} (c) and (d)). 
% This behavior of the CNN was unexpected because there was no monkey face in the adversarial example at first glance.
% Thus, the expert examined the detailed neuron activations on this feature map and discovered that the high activations appeared in the top right corner of the neurons, which corresponded to the top right corner of the image (Fig.~\ref{fig:case0_monkey} (e)).
% The expert did not understand why the CNN detected a monkey face at that part of the image.
% By carefully examining the adversarial example and the learned features of the neurons, he finally figured out the reason: there is a dark strip with a bright strip on each side (Fig.~\ref{fig:case0_monkey}A).
% It is a recognizable attribute for the face of a guenon monkey, which made the CNN mispredict the adversarial example as a monkey.

% \subsubsection{Analyzing Black-box Adversarial Examples}

% % \noindent \textbf{\normalsize Data.}
% % Same as the data in the above case study.

% \noindent \textbf{\normalsize Model.}
% We used the VGG-16~\cite{simonyan2014very} network to analyze black-box attacks because our employed attacking method has the knowledge of a set of state-of-the-art CNNs, such as ResNet~\cite{He2016_CVPR_residual} and the Inception network~\cite{szegedy2016rethinking}.
% Thus, we adopted a traditional CNN (VGG) to analyze black-box attacks. 
% We utilized the pre-trained VGG-16 network from TensorFlow~\cite{Tensorboard2017_web}.
% It achieved a $84.8\%$ accuracy on the normal examples, and a $22.4\%$ accuracy on the adversarial examples.
% % Image preprocessing follows the approach recommended in TensorFlow.

% \noindent \textbf{\normalsize Analysis process.}
% The expert continued to explore the analyzed adversarial example, and tested it on the VGG network.
% He found that it was misclassified as a beagle (a type of dog, Fig.~\ref{fig:case2_dog} (a)).
% %It indicated that the black-box attack is successful for this image.
% To check how the prediction was made, the expert extracted and compared the datapaths for normal beagle images and  the adversarial panda image.
% He found that the there was no obvious ``merging point'' in VGG-16, because these images do not truly ``merge'' due to the high prediction score of beagle images (0.75$-$1.0) and the \shixia{relatively} low prediction score of the adversarial example (0.46). %because the activation similarity gradually decreased to 0 from the middle layers.
% Thus, the expert relied on his knowledge to select the layer that detected the highest-level features (Fig.~\ref{fig:case2_dog} (b)).
% By setting the color coding of feature maps as the activation of the adversarial example, the expert found a large activation appeared on a feature map in shared feature maps between the beagle's and adversarial panda's datapath (Fig.~\ref{fig:case2_dog}A).
% It is a potential cause that leads to the misclassification.
% Thus, he examined the learned feature of the neurons in this feature map (Fig.~\ref{fig:case2_dog} (c)), and found that they learned to detect the black nose of a beagle (a black patch, Fig.~\ref{fig:case2_dog}B).
% This feature is a recognizable attribute for a beagle.
% To understand why the adversarial example caused a large activation on this feature map, he further examined the activation heat map, and found that the neurons in the top right corner are highly activated (Fig.~\ref{fig:case2_dog}C).
% It indicates that there is such a feature in the corresponding part of the image.
% In particular, that part of the images is the black ear of the panda, which is also a black patch (Fig.~\ref{fig:case2_dog}C).
% This feature misled the VGG-16 network to detect a black nose in the adversarial panda image, which then led to the misclassification.

% \begin{figure}[htbp]
%   \centering
% %   \vspace{-2mm}
%   \includegraphics[width=\linewidth]{fig/case2_dog.pdf}
%   \vspace{-4mm}
%   \caption{The explanation of why the adversarial panda image was misclassified as a beagle (dog) by the VGG-16 network: (a) input images; (b) feature maps; and (c) neurons.}
%   \vspace{-4mm}
%   %(c) critical neurons found by our back-propagation based approach.}\looseness=-1
%   \label{fig:case2_dog}
% \end{figure}



==> TVCG-Analyzing the Robustness of Deep Neural Networks/background.tex <==
\section{Background}\label{sec:back}

In this section, we introduce how to generate adversarial examples.

==> TVCG-Analyzing the Robustness of Deep Neural Networks/conclusion.tex <==
\section{Conclusion}
We have presented a robustness-motivated visual analysis
\jw{tool, AEVis, to help} %approach that helps 
machine learning experts \jw{investigate the prediction process and understand the root cause 
\newdoc{%for
of} incorrect predictions of adversarial examples.} 
%understand the inner workings of adversarial examples and diagnose the root cause of incorrect predictions introduced by the adversarial \jw{noise.} %examples. 
%\jw{The key feature is the support of analyzing diverging-merging patterns between/among datapaths comparing datapaths of both adversarial and normal images to faciliate the anlysis of diverging-merging patterns between the two datapaths.}
\jw{The visualization at multiple levels, together with the constrained datapath extraction, allows efficient identification of critical layers from datapaths' diverging-merging patterns and 
\newdoc{%then
}critical neurons from the activation maps. The contribution analysis and the rich interactions further enable users to trace the root cause 
\newdoc{%for
of the} misclassification of adversarial examples.}
%and the contribution analysis, allows identifying the key diverging-merging patterns between/among datapaths, identifying the critical neurons for the patterns, and tracing the root cause for misclassification back to lower layers.}
%The major feature of this approach is that it centers on the concept of datapaths to tightly combine datapath extraction and visualization. 
 \jw{We conducted a quantitative experiment to evaluate the datapath extraction method and a representative case study with an expert to demonstrate the usefulness of AEVis 
 \newdoc{%for
 in} explaining the reasons behind \newdoc{the} misclassification of adversarial examples.}
%Two case studies were conducted with two machine learning experts to demonstrate the effectiveness and usefulness of our approach in analyzing both white-box and black-box adversarial examples. 

\jw{There are several directions 
\newdoc{%to
we could} follow in our future 
\newdoc{%work
research}. First, based on the discovered root cause for misclassification, an interesting and important step forward is to develop targeted defense solutions. We will continue working with \newdoc{%the
}machine learning experts 
\newdoc{%, and
to} explore an effective route from discovered cause to targeted solutions for developing more adversarial robust DNN models. 
Second, complementary to developing defense solutions, another avenue is to detect potential adversarial examples online and remove them from further processing. A set of streaming visualizations that can incrementally integrate the incoming log data with existing data is the key to online monitoring.
Third, as discussed in Sec.~\ref{sec:discussion}, an interesting direction is to generalize AEVis to analyze the noise robustness of other types of DNNs, and to \keleiReRe{tackle} other types of data. 
\newdoc{%To improve
Improving} the scalability to deeper DNNs and the visualization of more datapaths is also 
\newdoc{%on this avenue.
an area of future interest.}
Different datapath extraction algorithms and suitable visualization designs would be 
\newdoc{interesting} research topics.
\newdoc{%following this direction.
}}

%One interesting avenue for future \doc{research} is to monitor the online testing process, detect potentially adversarial examples, and remove  them from any further processing. 
%work
%The key is to design a set of streaming visualizations that can incrementally integrate the \doc{incoming} log data with \doc{existing data}. 
%the existing one new coming
%We would also like to continue working with the machine learning experts to conduct several field experiments, \doc{with the aim of} designing  more targeted and effective defense solutions based on the discovered root cause. 
%which aims at 
%Another important direction is to analyze the robustness of other types of DNNs, such as RNNs and DGMs. 
%For these types of DNNs, exciting research topics include more efficient datapath extraction algorithms and suitable visualizations  for different types of DNNs. 

==> TVCG-Analyzing the Robustness of Deep Neural Networks/datapath.tex <==
\section{Datapath Extraction}
\label{sec:datapath}

% \begin{figure}[!t]
%   \centering
%   \vspace{-3mm}
%   \includegraphics[width=\linewidth]{fig/datapath_result.pdf}
%   \caption{A misleading result of the activation-based datapath extraction approach: (a) the input image; (b) the top 2 critical neurons found by the activation-based approach.
%   The learned feature is computed by the discrepancy maps~\cite{zhou2014object} and the activation heat map show the activations on the corresponding feature map.}
%   \label{fig:datapath_extraction_moti}
%   \vspace{-4mm}
% \end{figure}


\subsection{Basic Problem Formulation}

\mc{Extracting datapaths of adversarial and normal examples is the basis for analyzing why an adversarial example is 
%\newdoc{%is has been} 
misclassified (\textbf{R1}).
The key challenge is to identify the critical neurons in the prediction process. \jw{Once the critical neurons 
\newdoc{%being
have been} identified, selecting the corresponding connections to form the datapath is straightforward.} %as selecting the corresponding connections to form the datapath is straightforward.
}
%Such 
Critical neurons are \jw{those} %the neurons 
that highly contribute to the final prediction.
In other words, by only combining \jw{the critical neurons and corresponding connections,} 
%the contributions of the critical neurons, 
the prediction of an example will not be changed. %To this end, 
\jw{Therefore,} we aim 
\newdoc{%at selecting
to select} a minimized subset of neurons \jw{that can} %, which 
\newdoc{%keep
maintain} the original prediction. 
Accordingly, we formulate critical neurons extraction as a subset selection problem:
\begin{equation}
\label{eq:dp-ext2}
N^{opt}=\underset{{N_s}\subseteq N}{\mathop{\arg \min }}\,(p(x)-p(x;{N_s}))^2 +\lambda|N_s|.
\end{equation}
The first term is to keep the original prediction, and the second term ensures 
\newdoc{%to select
the selection of} a minimized subset of neurons.
Specifically, $N$ is the set of neurons in a CNN, $N_s$ is a subset of  %neurons 
$N$, $N^{opt}$ is the \jw{optimized subset consisting of} %calculated 
critical neurons, $p(x)$ is the prediction of example $x$, and $p(x;N_s)$ is the prediction if we only consider the neuron subset $N_s$.
To measure the difference between two predictions, we adopt the widely used $\ell_2$ norm.
$|N_s|$ is the size of $N_s$ and $\lambda$ is used to balance the two terms.
\mc{
Compared with our previous work, we change the second term from $|N_s|^2$ to $|N_s|$.
With
\newdoc{%such a
this} change, we are able to accelerate the
\newdoc{%whole
entire} optimization process by obtaining a minimized subset of neurons more easily according to the Lasso algorithm~\cite{tibshirani1996regression}.}
% The second term in Eq.~(\ref{eq:dp-ext2}) is $\ell_1$ norm instead of $\ell_2$ norm which was used in our previous work.
% Because $\ell_1$ norm is easier to obtain sparse solutions than $\ell_2$ (more 0 is included in the final optimization result),
% it is more efficient to eliminate unimportant neurons.
% }
%\todo{Discuss with Shixia: whether to mention we use l1 here instead of l2 in VAST18}
% \mc{Compared with our previous work, we use $\ell_1$ norm instead of $\ell_2$ norm to measure the size of selected subset of neurons, which aims at producing a sparser result.}


The large search space in Eq.~(\ref{eq:dp-ext2}) hinders \jw{a direct solution,} %us in directly solving it.
which is mainly due to a large number of neurons in a CNN (usually millions).
To reduce the search space, we utilize the weight-sharing property in CNNs~\cite{Lecun2015_Survey} and group neurons into a set of feature maps.
Specifically, in a CNN, neurons in a feature map share the same weights, and thus learn to detect the same feature.
%Utilizing 
\jw{Making use of}
\newdoc{%this
this} characteristic, we 
\jw{replace the problem of critical neuron selection with feature map selection and reformulate the problem as:} \looseness=-1
%formulate the feature map selection problem as
\begin{equation}
\label{eq:dp-ext-fm}
F_{opt}=\underset{{F_s}\subseteq F}{\mathop{\arg \min }}\,(p(x)-p(x;F_s))^2 +\lambda|F_s|,
\end{equation}
where $F$ is the set of feature maps in a CNN, \newdoc{and} $F_s$ is a subset of $F$.

\begin{figure}[bpht]
  \centering
%   \vspace{-3mm}
    % \vspace{3mm}
  \begin{overpic}[width=0.97\linewidth]{fig/datapath_randomness.pdf}
  \end{overpic}
  \caption{
  The cause of randomness in datapath extraction. (a) two feature maps detect the same feature (a deer head); (b) there are two %many 
  equivalent candidate datapaths 
%   \jw{for a given} adversarial image.
  for the deer image.
  }
  \label{fig:expr_randomness}
\end{figure}

\begin{figure*}[!t]
  \centering
%   \vspace{1mm}
  \begin{overpic}[width=\linewidth]{fig/workflow-analysis.pdf}
  \end{overpic}
  \caption{The analysis workflow of the diverging pattern. The brown color represents the first step analysis, and the purple color indicates the subsequent analysis, which is iterative.}
  \label{fig:analysis_flow}
\end{figure*}


\subsection{Constrained Datapath Extraction}


\mc{The above method is successful in extracting the critical feature maps for \textbf{one} example but sometimes
\newdoc{%introduces difficulty in
creates difficulty when} \textbf{comparing} datapaths of adversarial and normal examples, especially in 
\newdoc{%detecting the
the detection of} merging patterns~\cite{liu2018analyzing}.
After
\newdoc{%discussing
discussions} with the domain experts (E$_1$ and E$_2$) and conducting several experiments,
we find that the difficulty is mainly due to the randomness in datapath extraction.
Specifically, different feature maps in a CNN may have \jw{very similar} %nearly the same 
roles, i.e., detecting nearly the same features~\cite{liu2017VI_towards}.
It means that \jw{the optimized datapath for an individual adversarial or normal example may not be unique, given the many feature maps with equivalent roles.}}
\mc{
Thus, extracting a datapath can be treated as sampling one from \newdoc{%those
}equivalently good candidate datapaths, which introduces randomness in\newdoc{to} the datapath extraction.
Extracting datapaths that share common feature maps may lead to two feature map subsets
\newdoc{%without
that lack} common feature maps.   
As a result, we may over-estimate the difference between two extracted datapaths, which hinders the detection of the diverging and especially the merging patterns.}

\mc{To illustrate the above analysis, we trained a 6-layer CNN on the CIFAR10 dataset~\cite{Krizhevsky2009_Report}.
The network contains 5 convolutional layers and 1 fully connected layer.
After training, two equivalently good datapaths for a deer image (the difference between values of Eq.~(\ref{eq:dp-ext-fm}) is less than \kelei{$0.127$) \newdoc{%are
were} extracted}.
By examining the feature maps in the two datapaths, we found two feature maps that detected the same feature (a deer head, Fig.~\ref{fig:expr_randomness} (a)) but %they 
belong\newdoc{ed} to \newdoc{%the two
}different datapaths (Fig.~\ref{fig:expr_randomness} (b)).
%For further verification, we examined the corresponding activation heat maps and found that the input deer image is highly activated in its head region.
The above experiment illustrates that feature maps in a CNN may detect
the same feature and thus perform similar roles.
As a result, there is randomness in the datapath extraction process.
This randomness hinders the detection of diverging and merging patterns when comparing datapaths.}\looseness=-1

% As shown in Fig.~\ref{fig:expr_randomness}, a deer image as the input for a neural network, a part of most critical neurons that share the same weights are grouped as a feature map (Fig.~\ref{fig:expr_randomness}(a): feature map 48).
% With deactivating these neurons, we extract a new datapath of the same image and find another feature map (Fig.~\ref{fig:expr_randomness}(a): feature map 28) that have the similar mechanism, which also consists of a part of most critical neurons in new datapath.
% To adequately demonstrate the similarity of mechanisms between feature maps, we first compare the learned features and activation heat maps of the deer image.
% Two feature maps both focus the head of the deer in image.
% Further more, we collect most activated image patches (Fig.~\ref{fig:expr_randomness}(a)) for each feature map from training data.
% Two feature maps are both most activated by the head of deer.
% Based on the above comparison, it is evidently that two feature maps have similar mechanisms when the neural network infers the probability of this image.
% As a result, these two feature maps can be replaced with each other in the extracted datapath.}


% In our previous work, the neurons that highly contributed to the final prediction are selected as critical neurons to form the datapath.
% Consequently, it is formulated as a subset selection problem and our method effectively helps experts locate the "diverging point".

% \kelei{
% To make "merging point" emerge, we consult experts and find the reason that the randomness of datapath extraction prevent us from discovering the "merging point".
% It can be illustrated with a toy example in Fig.~\ref{fig:expr_randomness}.
% Given 
% To illustrate how "merging point" disappears due to the randomness of the extracted datapath, we adopt an sketch of a neural network (Fig.~\ref{fig:expr_randomness}(b)).
% }


To faithfully disclose the diverging and merging patterns,
%the key is \jw{to reduce} %reducing 
\keleiReRe{we need to reduce}
the randomness in \jw{datapath extraction.}  %extracting datapaths.
% As we discuss above, 
The randomness is mainly caused by
\newdoc{%no
the lack of} preference among the feature maps that detect the same features.
To tackle this issue, we introduce additional constraints into the datapath extraction process, to
\newdoc{%prefer extracting
prioritize the extraction of} datapaths that share common feature maps.

\mc{
Accordingly, the datapaths $F_{opt}^1, ..., F_{opt}^i,..., F_{opt}^n$ for examples $x^1,...,x^i,...,x^n$ are extracted by optimizing:
\begin{equation}
\label{eq:dp-ext-new-1}
F_{opt}^1, ..., F_{opt}^i,..., F_{opt}^n = \underset{{F_s^i}\subseteq F}{\mathop{\arg \min }}\,\sum_{i}{L^i}+
\gamma \sum_{i,j}{dis(F_s^i,\ F_s^j)},
\end{equation}
where the first term $L^i = (p(x^i)-p(x^i;{F_s^i}))^2 + \lambda |F_s^i|$ measures how good the datapath is for the i-th example $x^i$.
The second term $dis(F_s^i,\ F_s^j)$ \jw{is the distance to measure the difference between the datapaths for the i-th and j-th example, which is defined in Eq.~(\ref{eq:dp-ext-new-3}).}
%\todo{The distance is introduced in Eq.~\ref{eq:dp-ext-new-3}.}
%is a distance function to measure the difference between the datapaths for the i-th and j-th example.
Adding the constraint helps extract datapaths that share common feature maps.
$\gamma$ is used to balance the two terms.
% quality measurement for individual datapaths and the distance constraint .
% \todo{discuss with kelei, not sound here}
% The third term is for minimizing differences between the extracted datapath and given constraints.
Although this method is theoretically sound, in practice, we find %\newdoc{have} found 
that it
\newdoc{%was
is} difficult to maintain all the predicted labels of the examples, \jw{a fundamental requirement for explaining the prediction process.}
%If an extracted datapath is not able to maintain the predicted label of an example, it is useless in explaining the prediction process of that example.
% Such property is a fundamental assumption of datapath.
The root cause of the problem is the complexity in jointly finding optimized datapaths for different examples.
To solve this problem, we instead approximate the joint optimization into a chain of simpler conditional optimizations.
We first obtain the datapath for one example (e.g., the adversarial example to analyze) and iteratively obtain others by treating the previously calculated datapaths as constraints.
In particular, for the $i$-th example, we solve:
\begin{equation}
% \small
\label{eq:dp-ext-new-2}
F_{opt}^i= \underset{{F_s^i}\subseteq F}{\mathop{\arg \min }}\,L_i+
\gamma \sum_{j=1}^{i-1}{dis(F_s^i, F_{opt}^j)}.
\end{equation}}
% We follow the formulation in our previous work (the first and second term) for keeping the original prediction and minimizing the number of selected neurons.
% The third term is for minimizing differences between the extracted datapath and given constraints.
% Specifically, , and its element constraint $N^c$ is an extracted datapath of another example.
% $N$ is the set of all the neurons in target model. $N^s$ is a subset of $N$, and $N^{opt}$ is the set of selected critical neurons.
% $p(x)$ is the prediction of example $x$, and $p(x;N^s)$ is the prediction if we only consider the neuron subset $N^s$.
% $|N^s|$ is the size of $N^s$.


\mc{To efficiently solve the above subset selection problem, we approximate this NP-hard discrete optimization~\cite{cormen2009introduction} with a continuous optimization:
\begin{equation}
\label{eq:dp-ext-new-3}
\begin{aligned}
& \vecz{opt}^i = \underset{\vecz{}^i\in [0,1]^n}{\mathop{\arg \min }}\, L(x^i, \vecz{}^i) + \gamma \sum_{j = 1}^{i-1} dis(\vecz{opt}^j, \vecz{}^i), \\
& L(x^i, \vecz{}^i)) = (p(x^i)-p(x^i;\vecz{}^i))^2 + \lambda |\vecz{}^i|, \\
& dis(\vecz{opt}^j, \vecz{}^i) = ||\vecz{opt}^j - \vecz{}^i||_2,
\end{aligned}
\end{equation}
where $\vecz{}^i=[z^i_1, \cdots , z^i_n]$ and $z_k^i \in [0,1]$ is the contribution of the $k$-th feature map in the datapath of the $i$-th example $x^i$.
% The distance $dis(\vecz{}^j, \vecz{}^i)$ is defined as the l2-norm
%\todo{I'm not sure whether this claim is good. I prefer using hamming distance in the discrete form and approximate it into L2}
%\todo{For computational efficiency},
We apply the commonly-used $\ell_2$ norm to measure the difference between two datapaths (the second term in Eq.~(\ref{eq:dp-ext-new-2})).
Eq.~(\ref{eq:dp-ext-new-3}) is further solved by constructing and training a DNN \jw{as in}~\cite{wang2018interpret}.
In particular, we embed the variable $\vecz{}^i$ into 
the target DNN and train the network on the target adversarial/normal examples by stochastic gradient descent (SGD).\looseness=-1
}


% \kelei{
% Following the solution used in our previous work\cite{liu2018analyzing}, we group neurons into a set of feature maps, and then use a discrete variable $z_i \in \{0,1\}$ to represent whether the extracted datapath contains corresponding feature map.
% Utilizing this transformation, a datapath is mathematically represented as a vector $\boldsymbol{z}=[z_1, z_2, \cdots, z_n]$.
% Therefore, the original problem(Eq.~(\ref{eq:dp-ext-new-1})) is transformed into 0-1 programming problem:
% \begin{equation}
%     \label{eq:dp-ext-new-2}
% \begin{aligned}
% & Dis(\vecz{s}, \vecz{c}) = |\vecz{s} - \vecz{c}|
% \\
% & \vecz{opt} = \underset{\vecz{s}\in \{0,1\}^n}{\mathop{\arg \min }}\,(p(x)-p(x;\vecz{s}))^2 + \lambda |\vecz{s}|+ \gamma \sum_{c\in \pfhi}{|\vecz{s} - \vecz{c}|}
% \end{aligned}
% \end{equation}
% $n$ is the number of feature maps. $\vecz{opt}$ , $\vecz{s}$ and $\vecz{c}$ are the corresponding mathematical representation of $N^{opt}$ , $N^s$ and $N^c$.
% The distance function $Dis(., .)$ is designed to count the number of different elements between two datapaths,
% since we encourage the extracted datapath to be more similar with given constraints.
% After discussion with experts, the definition of distance function $Dis(.,.)$ is replaced with $\ell_2$ norm, since $\ell_2$ norm is powerful and widely used in continuous optimization to minimize the difference.
% }

% \subsection{Motivation and Problem Formulation}

% Extracting the datapath that are responsible for the prediction of a group of examples
% is the basis for analyzing why an adversarial example is misclassified (\textbf{R1}).
% The key challenge is to identify the critical neurons as selecting the corresponding connections to form the datapath is straightforward.

% Next we discuss how to extract the critical neurons for an individual example and then extend our approach to selecting critical neurons for a set of examples.

% A commonly used method is to treat the most activated neurons as the critical neurons~\cite{bilal2018convolutional,kahng2018acti}.
% However, this method may result in misleading results, especially when a highly recognizable secondary object is mixed with the main object in an image.
% For example, Fig.~\ref{fig:datapath_extraction_moti} shows the top 2 critical neurons found by such activation-based approach for a sheepdog image (Fig.~\ref{fig:datapath_extraction_moti} (a), employed network: ResNet-101~\cite{He2016_CVPR_residual}, image label: Shetland sheepdog).
% We can see that the second highly activated neuron learns to detect the head of a dog (Fig.~\ref{fig:datapath_extraction_moti} (b)), which is indeed critical for classifying a sheepdog.
% However, the most critical neuron learns to detect a ball (Fig.~\ref{fig:datapath_extraction_moti} (b)), which is not an important feature for classifying a sheepdog.
% Such a misleading result root in that the neurons have complex interactions with each other and the activations of the neurons are processed by a highly nonlinear function to generate the final prediction.
% Thus, highly activated neurons may not be the critical neurons for a prediction.
% Such critical neurons are the neurons that highly contributed to the final prediction.
% In other word, by only combining the contributions of the critical neurons, the prediction of an example will not be changed.
% To this end, we aim at selecting a minimized subset of neurons, which keep the original prediction.
% Accordingly, we formulate critical neurons extraction as a subset selection problem:
% \begin{equation}
% \label{eq:dp-ext2}
% N^{opt}=\underset{{N_s}\subseteq N}{\mathop{\arg \min }}\,(p(x)-p(x;{N_s}))^2 +\lambda|N_s|^2 .
% \end{equation}
% The first term is to keep the original prediction and the second term ensures to select a minimized subset of neurons.
% Specifically, $N$ is the set of the neurons in a CNN, $N_s$ is a subset of neurons $N$, $N^{opt}$ is the calculated critical neurons, $p(x)$ is the prediction of example $x$, and $p(x;N_s)$ is the prediction if we only consider the neuron subset $N_s$.
% To measure the difference between two predictions, we adopt the widely used L2-norm.
% $|N_s|$ is the size of $N_s$ and $\lambda$ is used to balance the two terms.\looseness=-1

% As discussed in Sec.~\ref{sec:require}, extracting the common datapath for a set of examples instead of an individual example can improve the representativeness of the extracted datapath (\textbf{R1}).
% A natural extension of Eq.~(\ref{eq:dp-ext2}) is minimizing the sum of the difference in the prediction of the example set $X$:   
% \begin{equation}
% \label{eq:dp-set}
% N^{opt}=\underset{{N_s}\subseteq N}{\mathop{\arg \min }}\, \sum\limits_{x_k \in X}{(p(x_k)-p(x_k;{N_s}))^2 +\lambda|N_s|^2}.
% \end{equation}
% Next, we discuss how to effectively solve this problem.
% For simplicity, we take Eq.~(\ref{eq:dp-ext2}) (critical neurons for one example) as an example to illustrate the solution.

% \subsection{Solution to Subset Selection}

% Directly solving the subset selection problem (Eq.~(\ref{eq:dp-ext2})) is time-consuming because: (1) it is an NP-complete problem and (2) the search space is prohibitively large due to the large number of neurons in a CNN.
% We therefore combine a divide-and-conquer approach with a quadratic optimization to reduce the search space and find a more accurate approximation.
% In particular, a divide-and-conquer-based \textbf{search space reduction} method is developed to reduce the large search space by splitting the subset selection problem into a series of separate subproblems and grouping the neurons into feature maps.
% As each subproblem is still NP-complete, we then employ the \textbf{quadratic approximation} to more accurately approximate each NP-complete subproblem as an easy-to-solve quadratic optimization by Taylor decomposition, and solve it based on back-propagation.

% \subsubsection{Search space reduction}

% A CNN is traditionally represented as a directed acyclic graph (DAG), where each node represents a neuron and each edge denotes a connection between nodes.
% A widely-used approach to accelerate DAG-related algorithms is processing the nodes layer by layer~\cite{liu2013storyflow,sugiyama1981methods}.
% Triggered by these algorithms, we split the original subset selection problem (Eq.~(\ref{eq:dp-set})) into a set of subproblems.
% Each selects the critical neurons in one layer:

% \begin{equation}
% \label{eq:dp-ext-layer}
% N^i_{opt}=\underset{{N_s^i}\subseteq N^i}{\mathop{\arg \min }}\,(p(x)-p(x;{N_s^i \cup N^{-i}}))^2 +\lambda^i|N_s^i|^2,
% \end{equation}
% where $N^i$ is the set of the neurons in layer $i$ and $N^{-i}$ is the set of all other neurons in the CNN except the ones in layer $i$.
% After solving all the subproblems, we aggregate all the sub-solutions $N^i_{opt}$ into the final critical neuron set $N_{opt} = \bigcup\limits_{i}{N^i_{opt}}$.

% Although dividing the original problem into a set of subproblems can largely reduce the search space, the search space of each subproblem is still large because a layer may contain more than one million neurons.
% Thus, we group neurons into a set of feature maps to further reduce the search space.
% In a CNN, neurons in a feature map share the same weights, and thus learn to detect the same feature.
% Utilizing this characteristics, we formulate the feature map selection problem as
% \begin{equation}
% \label{eq:dp-ext-fm}
% F^i_{opt}=\underset{{F_s^i}\subseteq F^i}{\mathop{\arg \min }}\,(p(x)-p(x;{F_s^i \cup F^{-i}}))^2 +\lambda^i|F_s^i|^2,
% \end{equation}
% where $F$ is the set of feature maps in a CNN, $F^i$ is the set of the feature maps in layer $i$, $F_s^i$ is a subset of $F^i$, and $F^{-i}$ is the set of all other feature maps in the CNN except the ones in layer $i$. 

% \subsubsection{Quadratic Approximation}

% Although we have reduced the search space from millions of dimensions (neurons in a layer) to thousands of dimensions (feature maps in a layer), it is still time-consuming to solve Eq.~(\ref{eq:dp-ext-fm}) because it is an NP-complete discrete optimization problem.
% To tackle this issue, we transform the discrete optimization into a continuous optimization problem.
% In particular, we reformulate Eq.~(\ref{eq:dp-ext-fm}) as:
% \begin{equation}
% \label{eq:dp-refor}
% \mathbf{z}_{opt}^i=\underset{z^i_j\in \{0,1\}}{\mathop{\arg \min }}\,(p(x)-p(x;\mathbf{z}^i))^2 + \lambda^i(\sum\limits_{j}{z^i_j})^2,
% \end{equation}
% where $\mathbf{z}^i = [z_1^i, ... , z_n^i]$ and $z_j^i$ is an indicator to represent whether the $j$-th feature map in layer $i$ is critical.
% If the feature map is critical, $z_j^i=1$, otherwise, $z_j^i=0$.
% Triggered by spectral clustering~\cite{ng2002spectral}, we approximate the discrete optimization with a continuous optimization by removing the discreteness condition $z_j^i \in \{0,1\}$ and allowing $z^i_j$ to take a value in $[0,1]$:
% \begin{equation}
% \label{eq:dp-cont}
% \mathbf{z}_{opt}^i=\underset{z^i_j\in [0,1]}{\mathop{\arg \min }}\,(p(x)-p(x;\mathbf{z}^i))^2 + \lambda^i(\sum\limits_{j}{z^i_j})^2,
% \end{equation}
% Eq.~(\ref{eq:dp-cont}) can be solved using gradient-based numerical optimization approaches such as the BFGS (Broyden$-$Fletcher$-$Goldfarb$-$Shanno) algorithm~\cite{wright1999numerical}.
% The gradient ${\partial p}/{\partial z_j^i}$ is calculated by back-propagation~\cite{goodfellow2016deep}.
% However, this method is computationally expensive because the gradient-based optimization is an iterative process where we have to calculate the gradients ${\partial p}/{\partial z_j^i}$ at each iteration.

% According to the calculation process of back-propagation, the deeper a CNN is, the longer it takes to compute the gradients.

% To tackle this issue, we approximate Eq.~(\ref{eq:dp-cont}) as a quadratic optimization where we calculate the gradients only once.
% Since $p(x) = p(\mathbf{a}_1,...,\mathbf{a}_n)$ and $p(x;\mathbf{z}^i) = p(z_j^i\mathbf{a}_1,...,z_j^n\mathbf{a}_n)$,
% we rewrite Eq.~(\ref{eq:dp-cont}) as a multivariate function.
% Here $\mathbf{a}_j$ is the activation vector of the $j$-th feature map produced by example $x$.
% The Taylor decomposition~\cite{rudin1964principles} is then used to decompose $p(x) - p(x;\mathbf{z}^i)$ into a linear form: 
% $p(x) -p(x;\mathbf{z}^i) \approx \sum\limits_{j}{ (1-z_j^i) \mathbf{a}_j \cdot  {{\left. \frac{\partial p}{\partial \mathbf{a}_j^i} \right|}_{\mathbf{a}}} } $, where $\mathbf{a} = [\mathbf{a}_1^i, ..., \mathbf{a}_n^i]$ and $\mathbf{x}\cdot \mathbf{y}$ represents dot product between two vectors $\mathbf{x}$ and $\mathbf{y}$.
% By substituting the above decomposition into Eq.~(\ref{eq:dp-cont}), we obtain a quadratic optimization:
% \begin{eqnarray}
% \label{eq:dp-final}
% \mathbf{z}_{opt}^i & = & \underset{z^i_j\in [0,1]}{\mathop{\arg \min }}\,(\sum\limits_{j}{ (1-z_j^i) \mathbf{a}_j \cdot  {{\left. \frac{\partial p}{\partial \mathbf{a}_j^i} \right|}_{\mathbf{a}}} })^2 + \lambda^i(\sum\limits_{j}{z^i_j})^2\\
% \label{eq:dp-final2}
% & = & \underset{z^i_j\in [0,1]}{\mathop{\arg \min }}\, \mathbf{z}^i(Q^i+ \lambda^i I)(\mathbf{z}^i)^T -2q\mathbf{q}^i \cdot \mathbf{z}^i,
% \end{eqnarray}
% where $\mathbf{q}^i = [\mathbf{a}_1^i \cdot {{\left. \frac{\partial p}{\partial \mathbf{a}_1^i} \right|}_{\mathbf{a}}}, \cdots , \mathbf{a}_n^i \cdot {{\left. \frac{\partial p}{\partial \mathbf{a}_n^i} \right|}_{\mathbf{a}}}]$, $q$ is the sum of $\mathbf{q}^i$, $Q=(\mathbf{q}^i)^T\mathbf{q}^i$ is a $n \times n$ matrix, and $I$ is a $n \times n$ identity matrix.
% Solving Eq.~(\ref{eq:dp-final2}) only needs to evaluate the gradients once.
% We use the BFGS algorithm to solve Eq.~(\ref{eq:dp-final2}).
% To control the scale of the two terms, the parameter $\lambda^i$ is set to $0.1/|F^i|^2$, where $|F^i|$ is the number of the feature maps in layer $i$.\looseness=-1

% In the same way, we obtain a solution for selecting critical feature maps for a set of examples (Eq.~(\ref{eq:dp-set})).
% Compared with Eq.~(\ref{eq:dp-final2}), there are two differences: (1) replacing $Q_i$ by $\sum{Q_k^i}$ and (2) replacing $q\mathbf{q}^i$ by $\sum{q_k\mathbf{q}_k^i}$, where $k$ is the index of the example in the example set.


==> TVCG-Analyzing the Robustness of Deep Neural Networks/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

AEVis can \jw{effectively} %better 
illustrate the prediction mechanism of adversarial examples and help discover the \jw{root cause} %vulnerable neurons 
\doc{that leads} to incorrect predictions. 
%leading
However, it \jw{still} %also 
has several limitations, which may shed light on future research \doc{directions}.
%In this section, we discuss scalability and generalization of AEVis. 

% \subsection{Scalability}

\noindent \textbf{Time complexity.} The datapath extraction usually takes a few minutes and is computed offline. \mcrev{The contribution analysis is the only part that cannot be pre-computed because the contribution is calculated based on the selected neurons.
It usually takes about $5$ seconds to calculate 
\newdoc{%such
the} contribution using SGD to solve Eq.~(\ref{eq:vis-partial-analysis-fm}).
\newdoc{%For acceleration
To accelerate the process}, we can use the quadratic approximation
\newdoc{%in
from} our previous work~\cite{liu2018analyzing}, which
\newdoc{%has better time efficiency
is faster} (computation time $<1s$) but
\newdoc{%worse analysis accuracy.
less accurate.}
\newdoc{%As
Since} our target users (machine learning experts) focus more on analysis accuracy, the SGD-based solution is set as default.
\newdoc{%The users
Users} can switch to the approximated contribution analysis in the interface.
}


\noindent \textbf{\normalsize Visual scalability}.
We have demonstrated that AEVis is able to analyze a state-of-the-art CNN (ResNet101), which has 101 layers and is much deeper than traditional CNNs (e.g., VGG-Net).
More recently, \jw{deeper CNNs with thousands of layers~\cite{He2016_CVPR_residual} have been developed.} 
%researchers have developed many deeper CNNs with thousands of layers~\cite{He2016_CVPR_residual}.
When handling such deep \jw{neural networks, the layers of interest at low levels of the hierarchy \jw{are difficult to} %cannot 
fit in one screen, even with the help of our segmented DAG.} %DNNs, 
%if an expert zooms in to low levels of the layer hierarchy, the layers of interest cannot fit in one screen, even with the help of our segmented DAG.
%To alleviate this issue, %we can 
%\jw{a possible solution is to}
\keleiReRe{A possible solution to alleviate this issue is to}
employ a mini-map to help the expert track \doc{the} current viewpoint, which has \newdoc{%been
}proven effective in TensorFlow~\cite{wongsuphasawat2018visualizing}.
% The dot plot is another factor that hinders AEVis from analyzing CNNs with thousands of layers.
% \doc{This is because} a layer group may contain hundreds of layers, and the height of the \doc{resulting} dot plot will be too large, which is a waste of screen space.
% To solve this problem, we can use non-linear dot plots~\cite{rodrigues2018nonlinear} to improve the scalability of AEVis.\looseness=-1


%In addition, even with the help of , all the layers cannot 
%To solve this problem, we can leverage 

% Currently, simply adding more layers to a deep model often leads to performance degradation due to over-fitting~\cite{He2016_CVPR_residual}.
% When researchers successfully solve this problem and design a deep model with thousands of layers
% To handle deep the visualization  



% \noindent \textbf{\normalsize Number of image sets.}
\mc{
Currently, we utilize a river-based visual metaphor to illustrate the diverging and merging patterns.
The layout of the datapaths is calculated 
\newdoc{%by
using} a rule-based method (Sec.~\ref{sec:vis-net}).
Such a design 
%echos
\keleiReRe{echoes}
the most common analytical task 
\newdoc{%that
when} three datapaths 
\newdoc{%are
need} to be compared (adversarial examples, the normal source examples, and the normal target examples).
If more datapaths are to be analyzed, an optimization-based layout method can be applied.
For example, we can minimize the mean-square-error between the vector of real datapath distances and their screen distances with a constraint \newdoc{so} that the order of real datapath distances
%are
\keleiReRe{is} maintained. 
The above optimization problem is convex (convex functions over convex sets) and guaranteed to achieve a global minimum.
As we have not observed such needs, we leave this method in the discussion here. 
Apart from the river-based visualization, the treemap-based visualization in the layer level is the other factor that limits the 
\newdoc{%capability of analyzing
ability to analyze} a lot of datapaths.
The intuitive treemap-based design is suitable for comparing several datapaths~\cite{alsallakh2014visualizing} and has been 
\newdoc{%proved to be 
proven} effective in the case studies.
We can further improve its scalability by adopting \newdoc{a} less intuitive but more scalable set \newdoc{of} visualization techniques, such as PowerSet~\cite{alsallakh2017powerset}.}

% and  to illustrate the overlapping relationship between/among datapaths.}
% Although researchers found that approximately four objects can
% be tracked in a visual comparison~\cite{intriligator2001spatial,wang2016topicpanorama,yantis1992multielement}, experts may have special needs of comparing a lot of datapaths.



\noindent \textbf{\normalsize Generalization}.
AEVis aims 
\newdoc{%at analyzing
to analyze} the adversarial examples for CNNs because most research on adversarial attacks focuses on generating adversarial images for CNNs.

In addition to attacking CNNs, there are several initial attempts to attack other types of DNNs~\cite{Akhtar2018_threat}, such as recurrent neural networks (RNNs), autoencoders (AEs), and deep generative models (DGMs).
In these types of DNNs, \jw{there are also neurons that are critical for predictions.}
%there are also datapaths.
For example, Ming et al.~\cite{ming2017understanding} demonstrated that some neurons in an RNN were critical for predicting the sentiment of a sentence, such as the neurons for detecting positive/negative words.
Such neurons and their connections form a datapath for an RNN.
Thus, %by extracting and visualizing datapaths, 
AEVis can be extended to help understand the root cause of adversarial examples for these DNNs.
%The idea of our datapath extraction can be directly used.
%To this end, we need to develop 
\jw{The main extension \newdoc{required} is the development of} suitable datapath extraction and visualization methods for different types of DNNs.
% Based on the extracted datapaths, we need to develop suitable visualizations for different types of DNNs.  
For example, to visualize the datapath of RNNs, we can first unfold the architecture of an RNN to a DAG~\cite{Goodfellow2016}, and then employ a DAG layout algorithm to calculate the position of each unfolded layer.   


In addition to images, \jw{there are adversarial attacks on other types of data~\cite{Akhtar2018_threat}}, 
%researchers try to generate adversarial examples for other types of data~\cite{Akhtar2018_threat}, 
such as adversarial documents and adversarial videos.
To generalize AEVis to \jw{different} %other 
types of data, we need to change the visual hint for neurons (learned features and activation maps) according to the target data type.
% the datapath view (Fig.~\ref{fig:teaser}) needs not to be changed.
% The major change will in 
For example, \doc{when} analyzing adversarial documents, we can use a word cloud to represent the `learned feature' of a neuron~\cite{ming2017understanding}, %in an RNN~\cite{ming2017understanding}.
%for
%In the word cloud, we 
\jw{and} select the keywords that strongly activate the neuron.



==> TVCG-Analyzing the Robustness of Deep Neural Networks/introduction.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Introduction}

\maketitle

%\mengchen{Deep neural networks (DNNs) have demonstrated significant improvements over traditional approaches in many artificial intelligence tasks~\cite{Lecun2015_Survey}, such as image classification~\cite{He2016_CVPR_residual} and language translation~\cite{Sutskever2014_NIPS_Sequence}.}

Deep neural networks (DNNs) have %recently 
demonstrated superior performance in many artificial intelligence applications, such as pattern recognition and natural language processing~\cite{Lecun2015_Survey,jiang2019recent,liu2017VI_towards}.
However, researchers have recently found that \jw{even} a %high accuracy DNN is
\jw{highly accurate DNN can be} vulnerable to carefully-crafted adversarial \xia{examples that} are intentionally designed to mislead a DNN into making incorrect predictions~\cite{choo2018visual,Dezfooli2017_CVPR_Universal, Nguyen2015_CVPR_Deep,szegedy2013intriguing,Zheng2016_CVPR}.
%\doc{into} make wrong 
For example, 
\jw{an attacker can make imperceptible modifications
\newdoc{%of
to} a panda image (from \pictag{I}{1} to \pictag{I}{2} in Fig.~\ref{fig:teaser-overview}) to mislead a state-of-the-art DNN model~\cite{He2016_CVPR_residual} to classify it as a monkey.}
%an attacker can modify an image of a panda (\pictag{I}{1} in Fig.~\ref{fig:teaser-overview}) slightly, even imperceptible to human eyes.
%However, the generated adversarial example (\pictag{I}{2} in Fig.~\ref{fig:teaser-overview}) is able to mislead a state-of-the-art DNN~\cite{He2016_CVPR_residual} to classify it as something else entirely (e.g., a monkey).
% \mengchen{because the DNN detects a monkey's face in the top right corner of the adversarial example (Fig.~\ref{fig:case0_monkey}A)}.
This phenomenon
\newdoc{%brings
creates} high risk
\newdoc{%in
when} applying DNNs to safety- and security-critical applications, such as driverless cars, face recognition ATMs, and Face ID security on mobile phones~\cite{Akhtar2018_threat}.
\mcrev{For example, researchers have recently shown that even the state-of-the-art public Face ID system can be fooled by using a carefully-crafted sticker on 
\newdoc{%the
a} hat~\cite{komkov2019advhat}.}
%To tackle this issue, there \doc{have been} some initial efforts in defending against adversarial examples~\cite{Cisse2017_ICML_parseval}.
%are 
%However, due to the limited understanding of the working mechanism of adversarial examples, the proposed defense strategies \doc{have} often \doc{been} very heavy, which usually leads to performance degradation.
%are
% \mengchen{For example, Dong et al. added a regularization to all the neurons in the layer that extracts the highest-level features.
% Although this defense approach can improve the robustness of a DNN, it causes a 4$\%$ drop in accuracy.
% %Finding the critical neurons in that layer and designing more targeted defense strategies will potentially decrease the performance degeneration.}
% Thus, there is a growing need to find the critical neurons and thus understand the primary cause of the wrong predictions introduced by adversarial examples~\cite{Akhtar2018_threat}, which \doc{can facilitate} experts to design more targeted and effective defense strategies.}
% Thus, there is a pressing need to understand the inner workings of adversarial examples
Thus, there is \jw{an urgent} %a pressing 
need to understand the prediction process of adversarial examples
and identify the root cause of incorrect predictions~\cite{Akhtar2018_threat, wang2018interpret}.
Such an understanding is valuable for developing adversarially robust solutions~\cite{Goodfellow2015_ICLR_explaining,liao2018defense,pang2018towards}.
% \mc{The key is to analyze the prediction  processes of adversarial and normal examples.
%\setlength{\textfloatsep}{10pt}
% In particular, the recent survey identifies two important %analysis goals
\newdoc{%The
A}
recent survey identifies two important
\jw{questions that require analysis}~\cite{Akhtar2018_threat}:
%\kelei{(Fig.~\ref{fig:intro-simple-adv})}:
(1) why similar images (e.g., adversarial and normal panda images) \textbf{\normalsize diverge} \jw{into} %to 
different predictions, and 
(2) why images from different classes (e.g., adversarial panda images and normal monkey images) \textbf{\normalsize merge} \jw{into the} %to the 
same prediction.


% \begin{figure}[!t]
%   \centering
%   \small
%   \begin{overpic}[width=0.85\linewidth]{fig/intro-simple-adv.pdf}
% %   \put(7, 23){\textsf{Panda}}
% %   \put(24, 43){\textsf{Perturbation}}
% %   \put(65, 30){\textsf{Monkey}}
%   \end{overpic}
%   %\vspace{-2mm}
%   \caption{A panda image with imperceptible perturbations is misclassified as a monkey.}
%   \label{fig:intro-simple-adv}
% \end{figure}

% \mengchen{In this paper, we present a visual analytics approach to 
% As currently, almost all research on ADV is focused on CNNs,
% We take one CNN as an example}
%\mc{To achieve the aforementioned analysis goals,} 
\jw{To give analytical answers to the questions,}
%there are two technical challenges.
\keleiReRe{we need to solve two technical challenges.}
% understanding and analyzing adversarial examples.
The first %challenge 
is \mc{\jw{to disclose} %disclosing
the prediction process of a DNN.
To this end, we need to extract the critical neurons and their connections that are responsible for the predictions of examples (Fig.~\ref{fig:system} (b)).
Such neurons and their connections form the datapaths of examples~\cite{wang2018interpret}.}
% delete the below setence
% Disclosing the datapath will help experts design more targeted defense approaches.
However, in a DNN, the neurons have complex interactions with each other~\cite{Bengio2013_PAMI_Representation}.
Thus, it is technically demanding to disentangle the roles of these neurons
\newdoc{%in the whole
within the entire} network and \shixia{extract the critical neurons to} form the datapath.
% \todo{Besides, interactions between datapath OR neurons share the same functions.}
% which neurons are responsible for the wrong prediction.
% Because there are often millions of neurons in a deep model and these neurons often influence each other, accurately and effectively finding such neurons are technically demanding.
% For brevity, we denote the set of such neurons as the \textbf{datapath} and the first challenge can be abbreviated as \textbf{datapath extraction}.
%The second challenge is effectively visualizing datapaths.
The second challenge is to effectively illustrate \mc{and compare the prediction processes of adversarial and normal examples based on the extracted datapaths.}
% the inner workings of adversarial examples based on the extracted datapaths.
%an effective exploration mechanism for experts to examine and compare the datapath
%With the development of more effective training approaches, CNNs are becoming more complex.
A state-of-the-art DNN usually contains hundreds of layers, with millions of neurons in each layer~\cite{He2016_CVPR_residual}.
%Ori: First, a CNN may consist of tens or hundreds of layers (depth), with thousands of neurons (width) in each layer, as well as millions of connections between neurons
Thus, an extracted datapath potentially contains millions of neurons and even more connections.
%Moreover, a feature map usually contains thousands of neurons.
Directly visualizing all the neurons and %the corresponding 
connections in \mc{the extracted datapath} will \jw{result in} %lead to 
excessive visual clutter.\looseness=-1
%Ori:Directly visualizing all the time series with a line chart will induce excessive visual clutter

% multi-level
% many neurons
\mc{To tackle these challenges, we have developed a visual analysis tool, AEVis, to \jw{help identify} the root cause of \jw{misclassification of} adversarial examples.
Fig.~\ref{fig:teaser-overview} shows an example of using AEVis to analyze why an adversarial panda image is misclassified. 
On the one hand, we find that the extracted datapaths of the adversarial and normal panda images start to diverge at layer \kelei{\pictag{L}{A} (Fig.~\ref{fig:teaser-overview})} and eventually lead to 
different predictions.
On the other hand, merging starts at layer \kelei{\pictag{L}{C} (Fig.~\ref{fig:teaser-overview})} in the datapaths of %monkey images and 
the adversarial panda \jw{and monkey images}. 
With the \jw{use of the developed} %help of our 
multi-level visualization, we identify the root cause of this misclassification as 
\jw{both a failed detection of the outline of \newdoc{one of} the panda's
\newdoc{%one ear
ears} and a faulty detection of a monkey face in the adversarial panda image using the target DNN.}
%that the target DNN detects a monkey's face in the top right corner of the adversarial panda image.
}\looseness=-1
%\todo{modify after the case study}

\mc{Technically, AEVis aims to disclose the prediction process of a DNN by extracting and visualizing \jw{the} datapaths for adversarial and normal examples, especially focusing on illustrating how \jw{these} datapaths \jw{diverge and merge.} %merge and diverge.
}

\mc{To achieve 
\newdoc{%the
this} aim, 
% we have first developed a datapath extraction \jw{algorithm} %approach 
% that discloses the prediction process of a DNN.
we first formulate the datapath extraction as a subset selection problem, which aims
\newdoc{%at selecting
to select} a minimum set of neurons that can maintain the predictions of a set of examples. 
As neurons in a DNN sometimes have similar roles, 
\jw{there is randomness in selecting neurons in the datapath extraction process.} 
\jw{As a result, the uniqueness of an example's extracted datapath cannot be guaranteed.}  %the datapath of a set of examples is not unique.
% Thuextracting datapaths of adversarial and normal images independently will
%Thus, extracting a datapath can be treated as sampling from a pool of equivalently good candidate datapaths, which introduce randomness in the extraction process.
\jw{Moreover,} the randomness hinders the detection of the diverging and merging patterns \jw{in} %of 
the extracted datapaths.
% , while maintaining the diverging/merging patterns of the extracted datapaths.
To reduce the randomness, we %add a 
\jw{introduce the} 
constraint that 
\newdoc{%the
it is desirable for the} datapaths of adversarial and normal examples
\newdoc{%are desired
}to share common feature maps (\todo{a set of neurons that share the same weights in a DNN}).   
% we simultaneously extract the datapaths for both adversarial and normal examples as well as add a soft constraint to the distance between the datapaths of adversarial and normal examples.
To extract the datapath\newdoc{s} for large DNNs, we approximate the subset selection problem as a continuous optimization 
%The continuous optimization problem is 
\jw{that can be} efficiently solved by constructing and training a neural network~\cite{wang2018interpret}.}
% We find that the key of disclosing the divergin/merging patterns is to reduce the 
% To effectively solve the problem, we construct and train a neural network}

\mc{Second, we have developed a multi-level visualization that illustrates how the extracted datapaths diverge and merge in the prediction process.
In particular, at the network-level, we 
\newdoc{%develop
have created} a river-based visualization to provide an overview of the diverging and merging patterns of datapaths.
At a detected diverging/merging point (layer level), we employ a treemap-based set visualization to  %illustrate critical neuron groups belonging to different datapaths, 
\jw{illustrate the neuron groups at this layer and their
belonging to different datapaths.} 
\jw{This} %which 
helps experts determine the critical \jw{neurons} %neuron groups 
that cause %responsible for 
the diverging and merging patterns.} %point.}
% The \jw{activation of neurons} %detailed neuron activation 
% is visualized in heat maps that are familiar to machine learning experts (neuron level).
% Between the layer level visualization and neuron level, we have added a feature map level because a layer may contain millions of critical neurons.
% A feature map is a set of neurons that share the same weight and thus detect the same feature.
% At the feature map level, 
\mc{In addition, we
\newdoc{%enhance
have enhanced} the multi-level visualization with a set of rich interactions that 
enable experts to effectively analyze \jw{the cause of diverging/merging of datapaths.} 
%why datapaths diverge/merge.
For example, we allow experts to interactively analyze the contribution of neurons in one layer to those of another deeper layer in order to disclose the root cause of a diverging/merging \jw{pattern} %point 
in the compared datapaths.}

The paper 
\newdoc{%extends
is an extension of} our previous work~\cite{liu2018analyzing}, 
\newdoc{%where
in which} datapaths of examples are extracted and illustrated.
In this paper, we
\newdoc{%solve
address} the problem 
\newdoc{%that
of} merging patterns
\newdoc{%are
that were} not detected in
\newdoc{%the
our} previous 
\newdoc{%work
method}.
We provide a better overview of diverging and merging between the datapaths of examples. 
In addition, the root cause of such patterns is analyzed
\newdoc{%deeper
more deeply} with our refined analysis workflow.
\mcrev{To evaluate the usefulness of the new system, we re-invited one expert in our previous work and conducted a deeper analysis of the same two adversarial image pairs, panda-monkey (Sec.~\ref{sec:panda}.1) and cannon-racket (Sec.~\ref{sec:cannon}.2).}
These improvements come from the following technical contributions:
% \mcrev{Compared with our previous work, we made the following technical contributions:}
%how datapaths of adversarial and normal examples \textbf{diverge} and \textbf{merge}, including:
\begin{compactitem}
\item\noindent{\textbf{\normalsize A constrained datapath extraction \jw{algorithm}%approach
} to extract datapaths while preserving their diverging and merging patterns.
% of the extracted datapaths.
}
\item\noindent{\textbf{\normalsize A river-based visualization} to provide an overview of how datapaths diverge and merge at the network level and \textbf{\normalsize a refined layer-level visualization} to reveal the feature maps of interest.}
% \item\noindent{\textbf{\normalsize A set of rich interactions} (e.g., contribution analysis of neurons between two layers) to help experts analyze the root cause of \jw{divergence/merging at certain layers.} %a diverging/merging point.
% }
\item\noindent{\textbf{\normalsize A contribution analysis method} to iteratively investigate the contribution of neurons between two layers and help experts analyze the root cause of diverging/merging
\newdoc{%at
in} certain layers.} %a diverging/merging point.
\end{compactitem}


% To tackle these challenges, we have developed a visual analytics tool, AEVis, to explain the root cause of the wrong predictions introduced by adversarial examples.
% The key is to effectively extract and understand the datapath of adversarial examples.
% We formulate the datapath extraction as a subset selection problem, which is NP-complete~\cite{cormen2009introduction}.
% To analyze the adversarial examples in large DNNs, we approximate the subset selection problem as \doc{an} easy-to-solve quadratic optimization by Taylor decomposition, and solve the quadratic optimization using back-propagation~\cite{christopher2006_PRML}.
% %a more 
% Based on the extracted datapaths, we design a multi-level visualization that enables experts to effectively explore and compare datapaths from the high-level layers to the detailed neuron activations.
% In particular, at the layer-level, we design a segmented directed acyclic graph (DAG) visualization to provide an overview of the datapaths.
% The detailed neuron activations are shown as heat maps that are familiar to machine learning experts (neuron level).
% %A dot plot is combined with the segmented DAG visualization, acting as a visual hint to enable experts select the layer of interest.
% Between the layer level visualization and neuron level, we \doc{have added} a feature map level because a layer may contain millions of critical neurons.
% %add 
% %An expert can select multiple layers and analyze the critical feature maps of these layers in more detail.
% A feature map is a set of neurons that share the same weight and thus detect the same feature.
% At the feature map level, we employ a tree map to illustrate and compare critical feature maps belonging to different datapaths.
% % The next sentence will be refined according to case study
% Two case studies are conducted to demonstrate that our approach can better explain the working mechanism of both white-box and black-box adversarial examples.
% , and thus can facilitate experts in designing a more robust DNN
% \mengchen{We conduct two case studies to demonstrate how our approach helps experts determine whether an image is an adversarial example or not, explain the wrong predictions introduced by such adversarial examples, and thus design more robust CNNs.}


% The key technical contributions of this \doc{paper} are:
% %work
% \begin{compactitem}
% \item\noindent{\textbf{\normalsize A visual analytics tool} that explains the primary cause of the wrong predictions introduced by adversarial examples.}
% \item\noindent{\textbf{\normalsize A datapath extraction method} that discloses critical feature maps and their connections that are responsible for a prediction.}
% \item\noindent{\textbf{\normalsize A multi-level datapath visualization} that enables experts to examine and compare datapaths, from the high-level layers to the detailed neuron activations.}
% %\item\noindent{\textbf{A credit assignment algorithm} that explains how the neurons contribute to a training failure.}
% \end{compactitem}

\todo{In this paper, we focus on analyzing adversarial examples generated for convolutional neural networks (CNNs), because CNNs are among the most widely-used networks, and most of the current adversarial example generation methods focus on attacking CNNs~\cite{Akhtar2018_threat}.
Our method can \newdoc{also} be 
\newdoc{%applied
used} to analyze adversarial examples
\newdoc{for} other deep networks that use CNNs as the key components.} 
% \jun{maybe better to change to: In this paper, we focus on analyzing adversarial examples generated for convolutional neural networks (CNNs), which are the most widely used networks. The techniques may be applied to analyze other deep networks that use CNNs as key components. 
% }

% Challenge:

% 1. Extract datapath: 
% 1.1 determine the contribution of a feature map to a classification result
% 1.2 determine the influence of a feature map to another (to mention DGMTracker?)

% 2. Visualize the datapath and how images "pass" the datapath
% 2.1 scalability: 100+ layers, 1000+ feature maps in one layer
% 2.2 compare datapaths to illustrate the difference between normal examples and adversarial examples


% 1. datapath generation
% Step 1: feature maps (or neurons?) based on LIME (KDD 2016)
% Step 2: also based on LIME
% %connections based on Taylor decomposition (or partial derivatives)

% 2. visualization
% Step 1: DAG
% Step 2: segmentation based on DP
% Step 3: neurons based on Euler diagram
% Step 4: connections based on biclustering 


% Contribution:

% 1. datapath generation
% 2. focus+context datapath visualization, combining DAG, DAG segmentation (partition?), Euler diagram, biclustering

==> TVCG-Analyzing the Robustness of Deep Neural Networks/related.tex <==
% !TEX root = EvoTree-KDD.tex


% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
%                                      & Network structure & No. instances visible         & Major goal                    \\ \midrule
% Network-centric methods           & Yes               & 0                             & Explore the network structure \\
% \textit{Instance-centric methods} & No                & Thousands $\sim$even millions & Analyze instance relations    \\
% Hybrid methods                    & Yes (as context)  & 1 $\sim$a few dozens          & Analyze prediction process    \\ \bottomrule
% \end{tabular}%
% }
% \caption{Connections and differences of network-centric, instance-centric, hybrid methods.}
% \label{tab:related}
% \end{table*}

\section{Related Work}\label{sec:related-work}

In the field of visual analytics, a number of methods have been developed to illustrate the working mechanism \kelei{of} a variety of DNNs, such as CNN~\cite{pezzotti2018deepeyes, nie2018tnnvis, bilal2018convolutional}, RNN~\cite{ming2017understanding, strobelt2018lstmvis, kwon2018retainvis, strobelt2018seq2seq}, deep generative models~\cite{liu2017analyzing, wang2018ganviz, Kahng2018ganlab}, and deep reinforcement learning models~\cite{wang2018dqnviz}.
Hohman et al.~\cite{Hohman2018VisualAnalyticsSurvey} presented a comprehensive survey to summarize the state-of-the-art visual analysis methods for explainable deep learning.
% using a human-centered interrogative framework.
Existing methods can be categorized into three classes:
network-centric~\cite{Liu2017_TVCG_Towards,Tzeng2005_VIS, wongsuphasawat2018visualizing}, instance-centric~\cite{rauber2017visualizing, bilal2018convolutional, wang2019deepvid, ma2019explaining}, and hybrid~\cite{Harley2015_ISVC,kahng2018acti}.\looseness=-1
% The connections and differences of the three kinds of methods are summarized in Table.~\ref{tab:related}.


\noindent\textbf{Network-centric methods.}
Network-centric methods help explore the
\newdoc{%whole
entire} network structure of a DNN, illustrating the roles of neurons/neuron connections/layers in the training/test process.
\newdoc{%As one of the 
In the} pioneering work, Tzeng et al.~\cite{Tzeng2005_VIS} employed a DAG visualization to illustrate the neurons and their connections.
% In this visualization, each neuron is represented by a node and their connections are represented by edges.
This method can illustrate the structure of a small neural network but suffers from severe visual clutter when visualizing state-of-the-art DNNs.
To solve this problem, Liu et al.~\cite{Liu2017_TVCG_Towards} developed a scalable visual analysis tool, CNNVis, based on clustering techniques. 
It helps explore the roles of neurons in a  %DNN 
\jw{deep CNN} and diagnose %a 
failed training processes.
Wongsuphasawat et al.~\cite{wongsuphasawat2018visualizing} developed a tool with a scalable graph visualization to present the dataflow %graph 
of a DNN.
To produce a legible graph visualization, they applied a set of graph transformations that converts the low-level \jw{graph of dataflow} %dataflow graph 
to the high-level structure of a DNN.

The aforementioned methods %facilitate experts in better understanding 
\jw{help experts better understand} 
the network structure, but they are less capable of explaining the predictions of individual examples.
% For example, the TensorFlow Graph Visualizer developed by Wongsuphasawat et al.~\cite{wongsuphasawat2018visualizing} does not extract and disclose the datapath of a set of examples, which is critical for identifying the root cause of the misclassification produced by adversarial examples.


\noindent\textbf{Instance-centric methods.}
% There are several recent attempts that centers at instances instead of the network structure.
To address the aforementioned issue,
%there are several recent attempts that center at instances.
\keleiReRe{researchers made several recent attempts that
\newdoc{%center at
focus on} instances.}
% These attempts aim at analyzing the relationships of the instances and the learning behavior of a DNN which is indicated in the instance relationships.
% These attempts aim at analyzing the relationships of the instances and the learning behavior revealed by the instance relationships.
These attempts aim at analyzing the learning behavior of a DNN revealed by the instances.
% To achieve this, a widely-used method is feeding a set of instances into a DNN, and visualizing their internal data, such as activations or the final predictions.
%To achieve this, a widely-used method is feeding a set of instances into a DNN, and
\keleiReRe{A widely-used method is feeding a set of instances into a DNN and}
visualizing \shixia{the corresponding log} data, such as the 
% \jw{activation maps} %
activation or the final predictions.
% We found that this hierarchy not only dictates the confusion patterns between the classes, it furthermore dictates the learning behavior of CNNs


For example, Rauber et al.~\cite{rauber2017visualizing} designed a compact visualization to reveal how the internal activation of training examples evolves during a training process.
They used t-SNE~\cite{maaten2008visualizing} to project the high-dimensional activation \jw{maps} of training examples in each snapshot 
\newdoc{%to
onto} a 2D plane.
The projected points are connected by 2D trails to provide an overview of the activation 
\newdoc{%in
during} the whole training process.
\mc{The method successfully demonstrated how different classes of instances are gradually distinguished by the target DNN.}
% and thus revealed the semantic similarities of these instances from the perspective of a target DNN.
\newdoc{%Besides
In addition to} internal activation, the final predictions of instances can also help experts analyze the instance relationships.
For example, the tool Blocks~\cite{bilal2018convolutional} utilizes a confusion matrix to visualize the final predictions of a large number of instances.
%To reduce the visual clutter caused by large number of instances and classes, the confusion matrix was enhanced by techniques such as
\keleiReRe{To reduce the visual clutter caused by a large number of instances and classes, researchers enhanced the confusion matrix
\newdoc{%by
using} techniques such as}
non-linear color mapping and halo-based visual boosting.
\mc{The enhanced confusion matrix was able to disclose the confusion pattern among different classes of instances and further indicated the learning behavior of a target CNN.}
%  a hierarchical confusion pattern among classes and further .
% The confusion pattern successfully 

The above methods can provide an overview of a large number of instances and help experts analyze their relationships.
However, the prediction process of individual instances is less considered.
Compared with these macro-level methods, our method focuses on the micro-level and targets \newdoc{%at
}the prediction processes of a set of instances (usually a few to dozens).
The prediction processes of these instances are visualized 
\newdoc{%by
using} a multi-level datapath visualization.
Revealing the prediction processes enables experts %in analyzing 
\jw{to analyze} the root cause of \newdoc{the} %misclassifications caused by the adversarial examples.
\jw{misclassification of adversarial examples.}\looseness=-1


\noindent\textbf{Hybrid methods.} The hybrid methods combine the advantages of network-centric and instance-centric methods.
Like instance-centric methods, the hybrid methods also feed the target instances into the network and extract log data such as activation \jw{maps}.
The extracted log data is often visualized in the context of the network structure, which provides visual hints to select and explore the data of interest, e.g., the activation in a specific layer.
Visualizing the log data in the context of network structure also helps experts explore the data flow from the network input to the output~\cite{liu2018steering}.

There are several 
\newdoc{%pieces of work
papers making progress} in this direction.
For example, Hartley et al.~\cite{Harley2015_ISVC} developed an interactive node-link visualization to show the activation in a DNN.
Although this method is able to illustrate detailed activation on feature maps, it suffers from severe visual clutter when dealing with large CNNs.
To solve this problem, Kahng et al.~\cite{kahng2018acti} developed ActiVis to interpret large-scale DNNs and their results.
They employed a multiple coordinated visualization to facilitate experts in comparing activation among examples.
The above works mainly focus on exploring the prediction process of \textbf{normal} examples.
\todo{Recently, there is an emerging need 
\newdoc{%from
in} safety-critical fields to analyze \textbf{adversarial} examples of DNNs.
While machine learning researchers have developed some holistic views on understanding the existence of adversarial examples~\cite{Goodfellow2015_ICLR_explaining, liao2018defense}, 
\newdoc{%there still lacks
there is still a lack of} visualization tools to analyze the details.}
\newdoc{%Echoing the
In response to this} need, we developed AEVis~\cite{liu2018analyzing} to analyze the root cause of misclassifications produced by malicious \textbf{adversarial} examples.
In particular, we developed a datapath extraction \jw{method} %method 
to extract critical neurons and their connections in the prediction process.
To enable experts \jw{to} explore the extracted datapaths, we designed a multi-level visualization that presented datapaths from the high-level network structure to the detailed neuron activation.

As an extension of our previous work~\cite{liu2018analyzing}, this paper %re-identified 
\jw{re-identifies} 
the central analytical task as analyzing the diverging and merging patterns of normal and adversarial examples.
Based on this task, we \jw{developed} %developed 
a constrained datapath extraction method that better \jw{preserves} %maintains 
the diverging and merging patterns of \newdoc{%the
}normal and adversarial examples.
% , thus better facilitates experts in comparing the prediction processes of these examples
We also 
\newdoc{%\jw{enhance} %enhanced
enhanced}
the whole analysis workflow by \jw{introducing} several useful interactions, such as \todo{activation analysis and contribution analysis}.
These interactions enable the experts to gradually investigate the major reason
\newdoc{%\jw{of}
for}
%that leads to 
this diverging/merging pattern and thus help them analyze the %misclassifications produced by 
\jw{misclassification of} 
adversarial examples.



%language inference model~\cite{liu2018nlize} 
%such as CNN (e.g., DeepEyes~\cite{pezzotti2018deepeyes}, TNNVis~\cite{nie2018tnnvis}, ~\cite{bilal2018convolutional, rauber2017visualizing}),
%RNN (e.g., RNNVis~\cite{ming2017understanding},  LSTMVis~\cite{strobelt2018lstmvis}, RetainVis~\cite{kwon2018retainvis}, Seq2Seq-Vis~\cite{strobelt2018seq2seq}),
%GAN (e.g., GANViz~\cite{wang2018ganviz},GAN Lab~\cite{Kahng2018ganlab}),
%deep generative model (e.g., DGMTracker~\cite{liu2018analyzing}),
%language inference model (e.g., NLIZE~\cite{liu2018nlize}) and
%reinforcement learning model (e.g., DQNViz~\cite{wang2018dqnviz}).
%Hohman et al.~\cite{Hohman2018VisualAnalyticsSurvey} \todo{(copy from its abstract) presented a survey of the role of visual analytics in deep learning research, which highlighted its short yet impactful history and thoroughly summarizes the state-of-the-art using a human-centered interrogative framework.}
%To illustrate the role of visual analytics in deep learning research, 
%A comprehensive survey on exploring the space of interpretability interfaces was presented by Olah et al.~\cite{olah2018building}.
%\kelei{Recently, Wang et al.~\cite{wang2019visualgenealogy} manually identified 66 representative DNNs and developed \todo{(copy from its abstract) an interactive visualization tool that offered a visual summary of representative DNNs and their evolutionary relationships}.}
%Most recent methods on explainable deep learning can be categorized into two groups: network-centric~\cite{Liu2017_TVCG_Towards,Tzeng2005_VIS, wongsuphasawat2018visualizing} and example-centric methods~\cite{ming2018rulematrix, wang2019deepvid, Harley2015_ISVC,kahng2018acti}.

% \mc{
% which can be further divided into two categories: knowledge distillation and internal exploration(\todo{is this name "internal exploration" suitable?}).
% }
% The knowledge distillation methods use interpretable models to approximate predictive behaviors of DNNs.
%For example, given training data and a classifier (such as a CNN), Ming et al.~\cite{ming2018rulematrix} extracted decision rules that produced same predictions for training data, and designed a matrix-based visualization to help users navigate and verify the rules.
%Unlike these methods, which focus on explaining the behavior of approximate models, our method helps experts analyze the behavior of neurons in a DNN with a multiple level visualization.
% As to get a more understandable explanation,
% these methods concentrate on visualizing approximate models without showing the details inside the neural network.
% Therefore, they cannot go deep into the neural network to disclose the impact of adversarial examples, which is important for analyzing the root cause of the misclassification.

% Although ActiVis can show the causes for misclassification to some extent, it cannot be directly used to illustrate the primary causes of the wrong prediction caused by adversarial examples as it heavily relies on \doc{expert} knowledge to select \doc{which} layer to examine.
% In addition, we argue that purely relying on activation in one layer will result in misleading results (Sec.~\ref{sec:eval_dp}).
% To solve this problem, we propose \doc{combining} activation and gradients for selecting critical neurons at different layers, which are connected to form a datapath for the adversarial examples of interest.
% In addition, we integrate a DAG visualization with dot plots, which provide guided visual hints to help experts select the layer of interest.\looseness = -1

% Ming et al.~\cite{ming2018rulematrix} use decision rules to approximate the prediction of a classifier (e.g., a CNN),
% and designed a matrix-based visualization to help users navigate and verify the rules.
% Compared with a CNN, decision rules are much easier for users to understand.
% Similarly, Wang et al.~\cite{wang2019deepvid} employ a linear classifier to approximate an image classifier (e.g., a CNN) in the neighborhood of a single example.
% They normalize and visualize the weights of the linear classifier as a set of images, which clearly disclose the area of interest of the linear model.





%Their work is More relevant to our work

% network centric: visualizing neurons, connections, ... e.g., cnnvis, 

% 2. we provide whole data path instead of the XXX in one / several layer (not sure)

% 3. focus on robustness

% 4. scalability


% \subsection{Adversarial Attacks on Deep Learning}
% Adversarial attacks are a new research focus of DNNs~\cite{Akhtar2018_threat}. 
% Existing efforts mainly focus on the generation of adversarial examples~\cite{Dezfooli2017_CVPR_Universal, Nguyen2015_CVPR_Deep} and \doc{how to defend} against adversarial examples~\cite{Cisse2017_ICML_parseval,Zheng2016_CVPR}.

% The key of generating an adversarial example is to find a very small perturbation that can mislead DNNs into misclassification.
% Recently, researchers have proposed a variety of methods \doc{for} finding such perturbations, including the Fast Gradient Sign Method~\cite{Goodfellow2015_ICLR_explaining}, universal adversarial perturbation~\cite{Dezfooli2017_CVPR_Universal}, and DeepFool~\cite{Moosavi-Dezfooli2016_CVPR_Simple}.

% The generation of adversarial examples \doc{has triggered} researchers to develop several methods to defend against adversarial attacks.
% A natural defense is training a DNN \doc{using} adversarial examples (adversarial training)~\cite{Goodfellow2015_ICLR_explaining, szegedy2013intriguing}.
% Although adversarial training can defend the training adversarial examples, Moosavi-Dezfooli et al.~\cite{Dezfooli2017_CVPR_Universal} discovered that new types of adversarial examples can be generated to attack DNNs \doc{that have been trained in this way}.
% To tackle this issue, a more effective strategy is \doc{to change} the network structure to improve the defense against unseen adversarial examples.
% \doc{Adding} regularization to the corresponding layer(s) is one of the most commonly used \doc{methods for this}.
% The typical regularization methods include input gradient regularization~\cite{ross2017improving} and layer-wise Lipschitz regularization~\cite{Cisse2017_ICML_parseval}.
% For example, Cisse et al.~\cite{Cisse2017_ICML_parseval} added a layer-wise regularization to control to the global Lipschitz constant~\cite{Lipschitz_continuity} of a DNN, and thus increased the robustness of a DNN to \doc{defend against} small perturbations in the input space.
% However, due to the limited understanding of the working mechanism of adversarial examples, the above defense strategies are often very heavy, which usually leads to performance degradation for large, complex datasets such as ImageNet~\cite{russakovsky2015imagenet}.
% To solve this problem, we \doc{have developed} a visual analytics tool to explain the primary cause of the wrong predictions introduced by adversarial examples. 
% Based on a few vulnerable neurons identified by AEVis (Fig.~\ref{fig:teaser}A), machine learning experts can design more targeted and effective defense strategies.

==> TVCG-Analyzing the Robustness of Deep Neural Networks/system.tex <==
\section{The Design of AEVis}\label{sec:system}


\begin{figure*}[t]
  \centering
  \vspace{5mm}
  \begin{overpic}[width=0.95\linewidth]{fig/system-overview.pdf}
  \scriptsize
  \put(45.2, 55.2){\textsf{(a)}}
  \put(12, 55){\textsf{Input Images and the Target Model}}
  \put(25.5, 51.7){\textsf{DNN}}
  \put(38, 51.7){\textsf{Prediction}}
  \put(39, 45.4){\textsf{Panda}}
  \put(38.5, 36.4){\textsf{Monkey}}
  \put(4.5, 52){\textsf{Normal source image}}
  \put(4.5, 47.2){\textsf{Noise}}
  \put(4.5, 36){\textsf{Adversarial image}}
  \put(4.5, 33.5){\textsf{Normal target image}}
  %%%%
  \put(96, 55.2){\textsf{(b)}}
  \put(70, 55){\textsf{Datapath Extraction}}
  \put(76.5, 51.7){\textsf{DNN}}
  \put(89, 51.7){\textsf{Prediction}}
  \put(90.5, 45.4){\textsf{Panda}}
  \put(90, 36.4){\textsf{Monkey}}
  \put(55.8, 52){\textsf{Normal source image}}
  \put(55.2, 47.2){\textsf{Noise}}
  \put(55.8, 36){\textsf{Adversarial image}}
  \put(55.8, 33.5){\textsf{Normal target image}}
  \put(80, 24){\textsf{(c)}}
  \put(34, 23.8){\textsf{Datapath Visualization}}
  %\put(10, 28.3){\textsf{Network-level}}
  \put(13, 20.7){\textsf{Network-level}}
  \put(42, 20.7){\textsf{Layer-level}}
  \put(65, 20.7){\textsf{Neuron-level}}
  \put(84.1, 13.8){\textsf{Feedback}}
  \end{overpic}
  \vspace{-2mm}
  \caption{\jw{AEVis system overview.} (a) Input of the AEVis system; (b) the datapath extraction module; (c) the datapath visualization module that illustrates the extracted datapaths \jw{at the network-, layer-, and neuron-level.}}
  \label{fig:system}
  \vspace{-2mm}
\end{figure*}

% \subsection{Motivation}
The development of AEVis
\newdoc{%collaborates
was in collaboration} with the machine learning team that won \newdoc{%the
}first place in the NIPS 2017 non-targeted adversarial attack and targeted adversarial attack competitions, which aim\newdoc{ed} at attacking CNNs~\cite{dong2018boosting,NIPS2017_Challenge}.
Despite the promising results \jw{they achieved}, the experts found %that the research process was
\jw{the research process} inefficient and inconvenient, especially \jw{in terms of} the explanation of the model outputs.
In their research process, a \jw{key} %central 
step 
\newdoc{%is
was} \jw{to explain the misclassification} %explaining misclassification 
introduced by adversarial examples.
Understanding why an error has been made \jw{helps the experts identify the model weakness} 
%help the experts detect the weakness of the model 
and further design a more effective 
\newdoc{%attacking/defending
attack/defense} method.
%To this end, they 
The experts thus desire a tool that can assist them 
in understanding the prediction process of the target CNN.
% Such understanding usually comes from \textbf{\normalsize extracting} and \textbf{\normalsize examining} the critical neurons and their connections, which are referred to as \textbf{\normalsize datapaths} in their field~\cite{wang2018interpret}.}

% \mc{Take the analysis of an adversarial panda image as an example.
% As shown in \kelei{Fig.~\ref{fig:system}(a)}, the panda image \jw{with added adversarial noise} is misclassified as a monkey.
% %As the base of their analysis, 
% \jw{To understand this misclassification,} the experts usually first extract the critical neurons for \jw{the prediction} 
% %predicting the panda image 
% as a monkey.
% Such critical neurons \jw{can be} %are 
% obtained by selecting the most activated neurons~\cite{Zeiler2014_ECCV} or using the more advanced but slower gradient-based approach~\cite{wang2018interpret}.} 
% After extracting \mc{the critical neurons that form the} datapath, the experts examine \jw{the neurons} %them 
% to understand their roles for \jw{the} prediction.
% Currently, they utilize discrepancy maps~\cite{zhou2014object}, heat maps~\cite{Zeiler2014_ECCV}, and weight visualization~\cite{Goodfellow2015_ICLR_explaining} to understand the roles of \mc{neurons and their connections in} the datapaths.
% Although these methods can help the experts at the neuron level, they commented \jw{the lack of} 
% %that there lacked 
% an effective exploration mechanism \jw{that can enable} %enabling 
% them to investigate the extracted datapaths from \mc{a network overview} to \mc{detailed} individual neurons.
% \mc{In addition to examining the datapath of the adversarial example, 
% \jw{the experts often find the need to compare the datapath of the adversarial example with those of the normal images, e.g., the normal panda and the normal monkey images.} 
% %the expert often put the datapath of the adversarial example in the context of normal images by comparing the datapath with the ones of normal images, e.g., the datapath of normal panda images and the datapath of normal monkey images.
% \jw{These comparisons can} 
% %Such comparison is able to 
% help them analyze (1) why similar images (adversarial and normal panda images) have different predictions and (2) why images from different classes (adversarial panda images and normal monkey images) have the same prediction.
% Currently, the comparison is done by %calculating and 
% manually examining the unique and shared critical neurons of different datapaths.
% This process involves a large amount of manual work (e.g., browsing the unique neurons one by one) and is thus inefficient.}

% \mc{To facilitate the above analysis process 
% and \jw{improve its efficiency,} %alleviate the inefficiency in it, 
% we collaborated with the experts \jw{and developed AEVis to allow} %to develop AEVis that allows 
% experts interactively analyze and compare the datapaths of the adversarial examples and normal examples.}
% \mc{To this end, they desire to understand: (1) why similar images (e.g., adversarial and normal panda
% images) have different predictions and (2) why images from different classes (e.g., adversarial panda images and normal monkey images) have the same prediction.}
% To this end, they desire to understand the roles of the neurons and their connections for prediction.
% Because there are millions of neurons in a CNN, examining all neurons and their connections is prohibitive.
% In the prediction of a set of examples, the experts usually \textbf{\normalsize extract} and \textbf{\normalsize examine} the critical neurons and their connections, which are referred to as \textbf{\normalsize datapaths} in their field.

% To extract datapaths, the experts often treat the most activated neurons as the critical neurons~\cite{Zeiler2014_ECCV}.
% However, they are not satisfied with the current activation-based approach because it may result in misleading results.
% For instance, considering an image with highly recognizable secondary objects, which are mixed with the main object in the image.
% The activations of the neurons that detect the secondary objects are also large, however, the experts are not interested in them because these neurons are often irrelevant to the prediction of the main object.
% Currently, the experts have to rely on their knowledge to manually ignore the neurons in the analysis process.\looseness=-1



%the consistency of the features learned by the neuron
% In particular, they can calculate the LC metric~\cite{dong2017towards} for a neuron to measure the consistency of the features learned by the neuron, compute discrepancy maps~\cite{zhou2014object} to understand the learned features of a neuron, show activations as heat maps to analyze the dataflow on a feature map~\cite{Zeiler2014_ECCV}, and use weight visualization to illustrate the interactions among several neurons ~\cite{Goodfellow2015_ICLR_explaining}.
% rely on high-level statistics, such as LC metric~\cite{dong2017towards}, and visualizations, such as the activation heat map~\cite{sabour2015adversarial} and the .

%Mengchen comment: whether to comment on current vis tools.  

% In summary, the experts desire a tool that can more accurately extract critical neurons and their connections, as well as allowing them explore them more effectively. 



% Their research process can be summarized as a loop between two steps:

% \noindent{\textbf{\normalsize Step 1}: explaining current results, e.g., why an adversarial image containing a panda is classified as a monkey.}

% \noindent{\textbf{\normalsize Step 2}: trying more advanced attacking/defending approaches, e.g., adding a regularization term in the loss function.}

% As there are usually millions of neurons in a layer, it is time-consuming to examine all neurons.
% Currently, they usually first aggregate neurons into hundreds of feature maps and select the critical feature maps for the prediction.

% with the highest activations.
% Such approaches are also widely used in current visual analytics tool for illustrating DNNs.
% However, in the discussion with the experts, we find that such activation-based approach sometimes results in misleading information.
% Sometimes, the feature maps with high activations is not important for the prediction.
% For example, background and panda
% Thus, they desire a better approach to extract the critical neurons and their connections.

% use some visualizations, such as heat map and discrepancy map to understand the activations and


% Currently, the inefficiency is largely caused by the explaining step (Step 1).
% In this step, they have to print a lot of high-level statistics, such as confidence scores and the LC metric.
% Based on these high-level statistics, they often select several layers and manually extract critical feature maps in these layers.
% To examine these critical feature maps, a density map and a discrepancy map are usually used to disclose the detailed activations on the interested feature maps and their learned features, respectively.
% Sometimes, they even have to putting some density maps and discrepancy maps side by side to compare multiple feature maps, which brings more mental burden.
% To make this step more efficient, the experts desire a tool that 
% can facilitate them in exploring the datapath in multiple levels.


%visually explain the classification result of a set of examples.

%providing an overview of the network and allowing them to gradually zoom in to details, such as the activations of neurons. 

% They desire a tool that support an exploratory analysis 
% They desire an exploratory analysis to help them explain their result and facilitate them develop more effective attacking/defending methods.  


\subsection{Requirement Analysis}
\label{sec:require}

% \mengchen{R1: extract the datapath of a set of examples 
% R2, Extract/Align/Match `` datapaths for adversarial and normal examples
% R3 Provide an overview of how datapaths diverge and merge.
% R4, Exploring datapaths at the detailed levels
% R2.5 Measure the distance between the datapaths.
% R5. Illustrating fm interaction.}

We have identified the following high-level requirements based on previous research and %the 
discussions with two experts (E$_1$ and E$_2$) from the winning team of the NIPS 2017 competition.

%\noindent \textbf{\normalsize R1 - Extracting the datapath for a set of examples of interest.}
\noindent \textbf{\normalsize R1 - \mc{Extracting the datapaths for adversarial and normal examples}.}
Both experts expressed the need for extracting the datapaths of \mc{adversarial} examples, \mc{which can disclose the prediction process of %an 
adversarial examples and thus} serves as the basis for analyzing why the adversarial examples 
\newdoc{%are
were} misclassified.
In a CNN, different neurons learn to detect different features~\cite{Zeiler2014_ECCV}, 
\jw{and play different roles} 
%Thus, the roles of the neurons are different 
for the prediction of an example.
% E$_1$ said that only analyzing the datapath can greatly save experts' effort %because they are able 
% \jw{to allow them} 
% to focus on critical neurons %instead of examining all neurons.
 E$_1$ said that only analyzing the datapath can greatly 
 \newdoc{%save experts' effort
 reduce their effort} by allowing them to only focus on critical neurons \jw{rather than \newdoc{having} to examine all of them.} 
% Besides the datapath for individual examples, E$_1$ emphasized the need for extracting the common datapath for a set of examples of the same class.
In addition to the datapaths for \mc{adversarial} examples, E$_1$ emphasized the need for extracting \mc{datapaths} for normal examples simultaneously.
\mc{He commented that as an adversarial example is often generated by slightly perturbing the pixel values of a normal image, \jw{there must be similarities between the two extracted datapaths.
Considering the similarity during the datapath extraction process will
%help extracting
\keleiReRe{help extract}
more meaningful datapaths for comparison \newdoc{%of the two
}during the analysis.}
%As a result, there should be some connections and regularities between the datapaths for normal examples and the corresponding adversarial examples.
%Such a connection is better to be considered in the datapath extraction process.
}
% He commented that the datapath of one example sometimes is not representative for the image class.
% For example, given an image of a panda's face, the extracted datapath will probably not including the neuron detecting the body of a panda, which is also a very important feature to classify a panda.

\noindent \textbf{\normalsize \mc{R2 - Comparing the datapaths of adversarial and normal examples.}}
\mc{As mentioned before, an adversarial example is often \jw{generated} %obtained 
by adding unperceivable noise to a normal example,} 
\jw{and thus
\newdoc{%has
there is} little difference from the normal image in the input space.} 
%Accordingly, a normal image and the corresponding adversarial example are nearly the same in the input space.
However, their prediction results are different.
The experts are interested in how they diverge \newdoc{in}to different predictions.
%For example, E$_2$ commented, ``I want to know whether there are some critical `diverging points' in a CNN or it happens gradually through the network.''
For example, E$_2$ commented, ``I want to know whether there are some critical `diverging points' for the \jw{different predictions} %prediction difference 
or 
\newdoc{%it is accumulated
they accumulate} gradually layer by layer through the network.''
To this end, E$_2$
\newdoc{%desired
wanted} to compare the datapaths of normal source examples and adversarial examples.
Triggered by E$_2$, E$_1$ added that it was interesting to compare the datapath of an adversarial example (e.g., a panda image that is misclassified as a monkey) with that of normal target examples (e.g., normal monkey images). 
Such comparisons help understand how these very different images ``merge'' into the same prediction (e.g., the monkey). 
The need for visual comparison is consistent with the findings of previous research~\cite{alexander2016task, gleicher2018considerations,liu2018visual}.\looseness=-1

% \noindent \textbf{\normalsize R2 - Providing an overview of the datapath.}
% \noindent \textbf{\normalsize \mc{R3 - Providing an overview of how datapaths diverge and merge.}}

\noindent \textbf{\normalsize R3 - Exploring datapaths at different levels.}
In a large CNN, a datapath often contains millions of neurons and connections.
Directly presenting all neurons in a datapath will induce severe visual clutter.
% Thus, it is necessary to provide experts an overview of a datapath.
E$_1$ commented, ``I cannot examine all the neurons in a datapath because there are too many of them.
%In the examining process, 
\jw{Instead,} I often start by selecting an important layer based on my knowledge and examine the neurons in that layer to analyze the learned features and the activation of these neurons.
%working mechanism of an adversarial example.
The problem %of this method 
is \newdoc{that} when dealing with a new architecture, I may not know which layer to start with.
Thus, I have to examine a bunch of layers, which is very tedious.''
%Thus, it is necessary 
\jw{He advocated \newdoc{for} the idea}
\newdoc{%to provide
of providing} %the experts 
an overview of the datapath with visual guidance to facilitate\newdoc{%s
} experts in selecting the layer of interest.
The requirement of providing an overview of a CNN aligns well with previous research~\cite{kahng2018acti,liu2018analyzing,wongsuphasawat2018visualizing}.
Although the overview of a datapath facilitates experts in finding the layer of interest, it is not enough to diagnose the root cause of the wrong prediction.
The experts said that %they wanted to link 
\jw{a 
\newdoc{%linkage
link} between} 
the overview of a datapath and the %with 
detailed neuron activation \jw{is required, which} 
%This linkage 
helps them identify the most important neurons that lead to misclassification.
% \mc{%To this end, 
\jw{To summarize,} 
it is
\newdoc{%desired
desirable} to provide a multi-level exploration mechanism that allows experts to zoom into the neurons of interest gradually.
% Since a layer may contain millions of critical neurons, the experts also desired a medium level between the layer level and neuron level.
% For CNNs, the experts recommended to group neurons into feature maps.
% E$_2$ said that, ``Neurons in a feature map learn to detect the same feature.
% Grouping them is very common in our research.''
Previous research also indicates that visual analytics for deep learning benefits from multi-level visualization~\cite{kahng2018acti,liu2018analyzing}.

\noindent \textbf{\normalsize R4 - \mc{Examining how neurons contribute to each other in a datapath}.}
Finding a diverging or merging point is not the end of the analysis.
To develop effective defense methods,
%it is critical to
\keleiReRe{we must}
disclose how such divergence or
\newdoc{%merge
merging} happens.
As the data flows from previous layers to the current diverging or merging point, a practical method of finding the root cause is tracing back to the previous layers and examining how \newdoc{the} neurons \jw{there} contribute to the neurons
\newdoc{%in
at} the diverging or merging point.
E$_1$ commented, ``When I find a neuron or feature map that performs very differently for an adversarial and a normal example, I'm interested in \jw{the cause of} 
\newdoc{%such
this} difference. 
For example, it is useful to know whether it \newdoc{was} caused by the neurons in the previous layer or even the neurons in a far-away layer due to the skip-connections~\cite{He2016_CVPR_residual} in modern CNNs.''
%To this end, 
\jw{Therefore,} we need to analyze how neurons contribute to each other in a DNN.
Previous research also indicates that presenting the contribution\newdoc{s} among neurons is \jw{important} %critical 
for understanding the outputs and roles of neurons~\cite{liu2018analyzing}.
% E$_1$ further commented that the .
% but how to enable a natural interaction to explore the interactions of interest because there are millions of or even billions of interactions between neurons. }





\subsection{System Overview}

Driven by the requirements
\newdoc{%collected from the
suggested by these} experts, we have developed a visual analysis tool, AEVis, 
% \mc{to help experts analyze and compare the prediction processes of adversarial and normal examples, which facilitates illustrating the root cause of \jw{the issues in robutstness to adversarial examples.}}
\mc{to help experts analyze the root cause of \jw{the 
robustness issues arising from adversarial examples.}}
%the robustness issues caused by adversarial examples.} 
% to illustrate the root cause of the robustness issues caused by adversarial examples.   
%motivated us to develop AEVis, which consists of the following modules:
It consists of the following two parts. 
\begin{compactitem}
\item\noindent{\textbf{\normalsize A datapath extraction module} that extracts the critical neurons and their connections for \mc{the predictions of adversarial and normal examples} (\textbf{R1}).}
\item\noindent{\textbf{\normalsize A datapath visualization module} that \mc{enables a multi-level (\textbf{R3}) visual comparison (\textbf{R2}) of the extracted datapaths and provides rich interactions (\textbf{R4}) to analyze the root cause of a misclassification}.} 
% \item\noindent{\textbf{\normalsize A datapath extraction module} that extracts the critical neurons and their connections for a set of selected examples (\textbf{R1}).}
% \item\noindent{\textbf{\normalsize A datapath visualization module} that provides an overall understanding of the datapath of interest (\textbf{R2}), illustrates datapaths in multiple levels (\textbf{R3}), and facilitates experts to visually compare several datapaths (\textbf{R4}).} 

%allow experts explore and compare datapaths from high-level layers to detailed neuron activations (\textbf{R2}, \textbf{R3}, \textbf{R4}).}
% Mengchen comment: whether to write this in more detail

% 
% \item\noindent{\textbf{\normalsize An interaction module} that provides a set of interactions such as comparing multiple datapaths (\textbf{R4}).}
\end{compactitem}

As shown in Fig.~\ref{fig:system} \todo{(a)}, AEVis takes a trained CNN and the examples to be analyzed as
\newdoc{%the
its} input.
The examples \mc{usually} include \mc{
the adversarial examples, normal source examples, and normal target examples.}
%both normal examples (Fig.~\ref{fig:system}A) and adversarial examples (Fig.~\ref{fig:system}B).
% Given the examples and the CNN, the datapath extraction module extracts the critical feature maps and their connections that are responsible for the predictions of the examples (Fig.~\ref{fig:system} (a)).
Given the examples and the CNN, the datapath extraction module extracts the critical \mc{neurons} and 
their connections that are responsible for the predictions of the examples (Fig.~\ref{fig:system} (b)).
The extracted datapaths are then fed into the visualization module (Fig.~\ref{fig:system} (c)), which supports the navigation and comparison of the datapaths from the high-level layers to the detailed neuron activation.\looseness=-1

% \todo{Needs to be justified by Kelei}
% \mengchen{A typical analysis workflow of AEVis is shown in Fig.~\ref{fig:teaser}.
% An expert explores the image list (Fig.~\ref{fig:teaser} (a)) and selects several groups of images for further understanding and analysis.
% After clicking on the `Analyze' button, AEVis first provides an overview of the datapaths at the layer level (Fig.~\ref{fig:teaser} (b)).
% At the layer level, each rectangle represents a layer group and a dot plot is combined with each layer group to illustrate the similarities between/among the extracted datapaths of the layers in each layer group.
% By examining the dot plots, the expert is able to detect layers of interest and further examines the feature maps in the layer ($L_C$ and $L_D$ in Fig.~\ref{fig:teaser}).
% In each layer, the Euler-diagram-based design helps the expert focus on the share/unique feature maps of several datapaths.
% % shows the overlapping relationship of the feature maps between/among the datapaths.
% Aided by this design and the color coding (e.g., activations) of feature maps, the expert can select a feature map of interest ($F_C$ and $F_D$ in Fig.~\ref{fig:teaser}), and explore the detailed neuron activations as well as the learned features of the neurons in this feature map (Fig.~\ref{fig:teaser} (c)).
% It facilitates him/her in finding the root cause (e.g., a set of neurons) for the misclassification of the adversarial examples.
% } 



% Experts can also interact with the generated visualization for further analysis.
% For example, experts can interactively select several groups of images and visually compare the datapaths of them.





==> TVCG-Analyzing the Robustness of Deep Neural Networks/visualization.tex <==
\section{Datapath Visualization}

\subsection{Overview}

An extracted datapath usually contains millions of neurons and even more connections,
% which prohibits experts from efficiently examining a datapath \mc{neuron by neuron} and \mc{comparing datapaths analyze the diverging and merging patterns}.
which prohibits %experts from 
efficient \jw{examination of the datapath or discovery of the merging-diverging patterns.} %examining a datapath neuron by neuron and \mc{discovering the informative diverging and merging patterns}.
% \mc{
% To help experts effectively explore and compare the extracted datapaths, we design a multi-level datapath visualization, which enables experts to analyze datapaths from high-level layers to detailed neuron activations (\textbf{R2}, \textbf{R3}, \textbf{R4}).
% Such multi-level visualization has been proved efficient in previous work on visual analytics of deep learning~\cite{liu2018analyzing} and echos the famous mantra ``overview first and details on demand.''}
To help experts systematically investigate the extracted datapaths, we \newdoc{have} design\newdoc{ed} a multi-level visualization to facilitate the datapath analysis from the high-level network structure to the detailed neuron activation (\textbf{R3}).
Accordingly, it consists of three major visualization components at the network-, layer-, and neuron-levels.

% Based on our discussions with the experts, we visualize datapaths on three levels: the network level, the layer level, and the neuron level.


% At each level, we (1) calculate the layout of the items (layers, feature maps, neurons) to reveal the relationships among them;
% and (2) provide visual hints to guide experts in finding the item(s) of interest and zooming in to a more-detailed level (e.g., from the layer level to the feature map level).

% Therefore, to enable an efficient exploration, we develop a a multi-level datapath visualization was proposed in our previous work to help experts analyze and compare datapaths on three levels (\textbf{R3}, \textbf{R4}): the layer level, the feature map level, and the neuron level (Fig.~\ref{fig:system}).
% }
% We continue to use a multi-level datapath visualization proposed in our previous work~\cite{liu2019analyzing} to help experts effectively explore the extracted datapaths,
% which enables experts to analyze and compare datapaths on three levels (\textbf{R3}, \textbf{R4}): the layer level, the feature map level, and the neuron level.
% To help experts effectively explore the extracted datapaths, we design a multi-level datapath visualization, which enables experts to analyze and compare datapaths from high-level layers to detailed neuron activations (\textbf{R2}, \textbf{R3}, \textbf{R4}).


%\subsection{Network-level Datapath Visualization}
\noindent \textbf{\normalsize Network-level visualization of data flows.}
 % \noindent \textbf{\normalsize Network-level.}
% At the network level, our primary goal is providing an overview of the extracted datapaths and disclosing the potential diverging and merging points.
% Our design is based on the fact that datapath is a subgraph of the target CNN (nodes: neurons, edges: neuron connections). 
% Currently, a widely-used approach to provide an overview of a CNN is formulating it as a DAG (directed acyclic graph) and using a node-link DAG visualization to present the network architecture~\cite{kahng2018acti,liu2018analyzing,wongsuphasawat2018visualizing}.
% Such an approach has been widely adopted by machine learning experts.
% To maintain this familiarity, we use the DAG visualization as the backbone of our network-level design.
% Specifically, we use the visualization method in the Graph Visualizer of Tensorboard~\cite{wongsuphasawat2018visualizing}.
% To solve the problem of very high aspect ratio when visualizing and exploring large CNNs (such as ResNet with 50-200 layers~\cite{He2016_CVPR_residual}), we develop a segmented DAG visualization inspired by the segmented timeline~\cite{brehmer2017timelines}.
% We transpose the vertical layout into a horizontal layout, segment the initial DAG into several parts, and visualize the segmented parts from top to bottom.
% The \textbf{network-level visualization} of data flows 
As shown in Fig.~\ref{fig:system} (c), the network-level visualization provides an overview of the extracted datapaths, discloses the potential diverging and merging points, and further guides experts in selecting a %diverging/merging point of interest (a layer in the network) 
\jw{layer of interest for examination} %to examine 
(\textbf{R2}).
\mcrev{Compared with our previous work, we replace %replaced %enhanced 
the dot-plot-based network-level visualization with %by 
a river-based visual metaphor, \keleiReRe{which has
%a
better scalability} and is more effective in depicting \newdoc{%the
} diverging and merging patterns.}
% When an expert detects a layer of interest, he/she is able to use the layer-level visualization to zoom in to the layer and examine the feature maps in the layer to grasp an idea of what feature maps are critical for the diverge/merge
% After a feature map of interest is observed, the expert can use the neuron-level visualization to explore the neurons in the feature map to analyze the root cause of the diverge and merge.
% Next, we will introduce the design of our multi-level visualization and how such design is made.

%We first illustrate how layers are connected.
% A widely-used approach is to formulate a CNN as a DAG (directed acyclic graph), where each layer is a node and their connections are edges~\cite{kahng2018acti,liu2018analyzing,wongsuphasawat2018visualizing}.
% Although the approach is available for large CNNs (such as ResNet with 50-200 layers~\cite{He2016_CVPR_residual}) with a hierarchy of the layers, when experts zoom in to the lower levels,
% the visualization suffers from a long skinny strip with a very high aspect ratio (Fig.8 (a) in~\cite{wongsuphasawat2018visualizing}).
% To tackle this issue, we develop a segmented DAG visualization inspired by the segmented timeline~\cite{brehmer2017timelines}.
% We transpose the vertical layout into a horizontal layout, segment the initial DAG into several parts,
% and visualize the segmented parts from top to bottom.
% The key challenge of our method is to decide where to segment a DAG,
% which is formulated as a ``printing neatly'' problem~\cite{cormen2009introduction}:
% \begin{equation}
% \label{eq:segment}
% \underset{e_i \geq 0}{\mathop{\min }}\, \sum\limits_{i=1}^{k-1}{e_i + \lambda c_i},
% \end{equation}
% where $k$ is the number of segments, $e_i$ is the empty space at the end of segment $i$, $c_i$ represents whether a building block is cut by segment  $i$.
% The first term is aimed at minimizing the sum of the empty space at the end of each line.
% To penalize a segmentation scheme that cuts a building block into two parts, we add a regularization term as the second term.
% $\lambda$ is used to balance the two terms.
% To guide experts to the interested layer,
% we further employ a dot plot as the visual statistical description of each layer,
% which is a compact visualization and widely used for relatively small datasets~\cite{rodrigues2018nonlinear}.

% \subsection{Layer-level Datapath Visualization}
\noindent \textbf{\normalsize Layer-level visualization of feature maps.}
 % \noindent \textbf{\normalsize Feature-map-level.}
When an expert identifies a layer of interest (e.g., a diverging or merging point), s/he then zooms in %to the layer 
to examine the critical feature maps in that layer (Fig.~\ref{fig:system} (c)).
For a diverging point, the unique feature maps of each datapath lie in the center of experts' analysis.
\newdoc{%As for
For} a merging point, the shared feature maps between/among datapaths are critical
\newdoc{%in
to} the analysis.
To help experts \keleiRe{
%\sout{better}
more} quickly find the important and informative feature maps,
%two types of filling styles are used
\keleiReRe{we use two types of filling styles}
to encode the activation \jw{difference} (solid filling $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_solid.pdf}}}$, Fig.~\ref{fig:system}A) and contribution (dotted filling $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_dotted.pdf}}}$, 
Fig.~\ref{fig:teaser-overview}$\textsf{F}_\textsf{A}$).
The higher filling %height 
represents a larger value.

% For example, given adversarial panda and monkey images, examining the shared feature maps in the datapaths is able to help experts analyze why the adversarial panda images are classified as monkey images.

% As finding unique/shared elements based on their set (datapath) membership is an important task tackled by the set visualization~\cite{alsallakh2014visualizing}, we then formulate the feature map layout problem as a set visualization problem.
% Among various set visualization techniques, such as the Euler diagram, the line-based techniques (e.g., LineSets~\cite{alper2011design}), and the matrix-based techniques (e.g., ConSet~\cite{kim2007visualizing}), we decide to employ on the Compact Rectangular Euler Diagram~\cite{riche2010untangling} (ComED) because: (1)
% % \begin{compactitem}
% It can well depict set relations and thus disclose the unique/share feature maps~\cite{alsallakh2014visualizing}; and (2) machine learning experts are familiar with Euler diagrams and they often use them to understand the set relationships.
% For example, feature map A in Fig.~\ref{fig:fm-layout-intro}(a) is a shared feature map of the three datapaths,
% while feature map B is a unique feature map for the yellow datapath.
% %\item The scalability is suitable in our scenario because experts usually compare no more than four datapaths at the same time;
% % \item The number of feature maps in each datapath is clearly conveyed in the Euler diagram, which is important for the analysis. 
% % \end{compactitem}}

%\begin{figure}[htbp]
%  \centering
%  \begin{overpic}[width=0.98\linewidth]{fig/fm-intro.pdf}
%  %{fig/visualization_feature-map-layout-intro.PNG}
%  %\put(0, 34.5){(a)}
%  \put(35, -3){(a)}
%  \put(49.5, 21){A}
%  \put(43, 16){B}
%  %\put(68, 34.5){(b)}
%  \put(81, -3){(b)}
%  \put(72, 17.7){1 FM}
%  \put(84.5, 17.7){2-9FMs}
%  \put(70.5, 3){10-99FMs}
%  \put(89, 10){...}
%  \end{overpic}
%  %\vspace{-2mm}
%  \vspace{2mm}
%  \caption{
%  Illustration on how to create a feature map visualization for three datapaths at a layer of interest. 
%(a) The three feature map sets of the datapaths at the selected layer;
%(b) The intersection relations among the sets;
%(C) Build a tree based on the set inclusion relations;
%(d) The treemap-based visualization of feature maps. The color of feature map encodes the activation or activation difference between two datapaths. The darker green indicates a higher value. }
%  \label{fig:fm-layout-intro}
%\end{figure}



% As in ComED~\cite{riche2010untangling}, we split the datapaths in the layer of interest by their intersection relations.
% This produces a hierarchy, which is visualized by non-overlapping rectangles (Fig.~\ref{fig:teaser-overview}$\mathrm{L_A}$).
% Then the split parts of datapaths are connected with lines, which can be shown on demand.
% Compared with ComED, we make two modifications to reduce visual clutter and better facilitate experts' visual comparison:
% \begin{compactitem}
% \item Utilize
% %K-Means~\cite{christopher2006_PRML}
% \kelei{agglomerative cluster method~\cite{ward1963hierarchical}} to cluster the feature maps by their activations to reduce the visual clutter caused by a large number of feature maps (Fig.~\ref{fig:fm-layout-intro}(b)).
% Experts can interactively modify the parameters of the clustering (e.g., the number of the clusters $k$) to reduce the parameter sensitivity.
% \begin{equation}
% \begin{aligned}
% \label{eq:treemap-optimization}
% & Cost = \sum_{S_i \in \{ 0,1\},\sum_i{S_i}\ge 2}
% (&
% Center(\mathop{\cap}\limits_{i:S_i=1}{A_i}) - & \\
% & & \mathop{Mean}\limits_{i:S_i=1}(Center(A_i)))^2 & 
% \end{aligned}
% \end{equation}
% \item Use the Treemap layout instead of the graph layout because the graph layout result has an irregular boundary, which is not suitable for juxtaposing multiple layers to compare the datapaths in them (Fig.~\ref{fig:teaser-overview}$\mathrm{L_A}$ and $\mathrm{L_C}$).
% \item Although we use clustering to reduce the visual clutter caused by a large number of feature maps, the layout becomes crowded when the number of subset increases (Fig.~\ref{fig:fm-layout-intro}(a)).
% A straightforward way to address this issue is using focus plus context technique.
% When an expert focus on one set, we maximize its region and minimize the regions of other sets.
% \kelei{Fig.~\ref{fig:teaser-overview}$\mathrm{L_C}$ and Fig.~\ref{fig:case-merging-overview}(c)(i) are examples that an expert focuses on different subsets in layer $L_C$ (Fig.~\ref{fig:case0_overview}).}
% \end{compactitem}

% % To illustrate such relationships, triggered by the Euler diagram~\cite{alsallakh2014visualizing}, we employ a treemap to illustrate the overlapping relationships between the datapaths.

% % To reduce the visual clutter caused by a large number of feature maps, we cluster the feature maps by their activations.

% To help experts efficiently select an interested feature map cluster, we encode the averaged importance/activation of each feature map cluster by its color (Fig.~\ref{fig:fm-layout-intro} (b)).
% Because experts usually start their analysis from the most critical or most highly activated feature maps.
% We also employ a series of stacked rectangles to represent a feature map cluster (Fig.~\ref{fig:fm-layout-intro} (b)).
% Triggered by Squares~\cite{ren2017squares}, the number of stacked rectangles encode the size of a cluster, which is proportional to the log of the cluster size.
% \subsection{Neuron-level Datapath Visualization}

% \begin{figure}[htbp]
%   \centering
% %   \vspace{1mm}
%   \begin{overpic}[width=0.7\linewidth]{fig/neuron-visualization.pdf}
%   \end{overpic}
%   \caption{Neuron-level visualization: (a) learned feature; (b) activation map.}
%   \label{fig:neuron_vis}
% \end{figure}

\noindent \textbf{\normalsize Neuron-level visualization of learned features.}
% \noindent \textbf{\normalsize Neuron-level.}
When an expert finds a feature map of interest,
% AEVis allows him/her to examine \mc{the details of the neurons of it} in the neuron panel (Fig.~\ref{fig:teaser-overview} (c)).
AEVis helps him/her understand what features the neurons of interest have learned in the prediction process.
% To preserve the visual link~\cite{Steinberger2011TVCG_link}, we add the same label to the feature map and the corresponding neurons(Fig.~\ref{fig:neuron_vis}A).
Following previous research~\cite{bilal2018convolutional, liu2017VI_towards}, we employ the learned features of the neurons $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_learned_feature.pdf}}}$ (Fig.~\ref{fig:teaser-overview}A) and their activation \jw{maps}  $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_activation_map.pdf}}}$ (Fig.~\ref{fig:teaser-overview}C) to facilitate the understanding.
% The activation of a neuron  or the activation difference between two datapaths is encoded by the color (green: positive activation). 
%need further modification - shixia
The activation of a neuron in a feature map is encoded by the color.
Darker green indicates a higher value.

\noindent\textbf{Analysis workflows}.
These three visualizations work together to support a progressive analysis of adversarial examples, which helps
\newdoc{%the expert
experts} understand the root cause of the \newdoc{%diverging
divergence} between normal source examples and the corresponding adversarial examples, as well as the merging between the adversarial examples and the normal target examples. 
Fig.~\ref{fig:analysis_flow} shows the typical \jw{workflow} %workflows 
for analyzing a diverging pattern. 
It starts from the network-level visualization where a diverging pattern (Fig.~\ref{fig:analysis_flow}A) with several layer groups is identified first. Then \newdoc{%by
%via
with} the layer-level visualization and activation analysis, the salient feature map is discovered.
Next, by analyzing the learned features and activation in the neuron-level visualization, the expert
\newdoc{%identifies
can identify} an area of interest in the focused feature map, which is sent to the contribution analysis module.
% This module computes the neuron contribution in the corresponding region of a feature map at previous layers to the activations of the selected neurons of the focused feature map.
% This module computes the corresponding neuron contribution of previous feature maps to the activations of the neurons in the focused region.
This module computes the contribution \jw{to the activation of the selected neurons} 
from corresponding neurons in previous feature maps. %to the activation of the neurons in the focused area.
Finally, by examining the contribution of the feature maps \jw{in} %belonging to 
the diverging pattern, the expert gradually investigates the major reason 
\newdoc{%that leads to
for} this \jw{divergence.} %diverging pattern.
In the merging pattern analysis, instead of using activation analysis, we use contribution analysis as the first step.
This is because the merging point is usually followed by the prediction. 
Contribution analysis helps identify \jw{the most important learned feature} %which learned feature is the most important one 
for the final prediction.
\mcrev{}

With this exploratory analysis, the potential \jw{cause} %account 
for the wrong predictions is disclosed to facilitate experts in their task of noise robustness analysis. 
In the below sections, we focus on introducing the network-level visualization, the layer-level visualization, and contribution analysis.
% The activation of a neuron is represented by its color (red: negative activation; green: positive activation).
% The neurons of a feature map are naturally organized on a grid,
% and their position are determined by the positions of the image patches that influence their activations~\cite{Goodfellow2016}.
% Combining the color coding and the grid-based layout of neurons, experts can detect which part of the image highly activates the neurons in the feature map.
% For example, in Fig.~\ref{fig:neuron_vis}B, we can find the neurons on the top right corner are highly activated, which corresponds to the panda ear in the image.
% To visualize the learned features of neurons, we employ the discrepancy map~\cite{zhou2014object} to highlight which region in the image actually highly activates a neuron and treat this region as the learned feature of this neuron.
% To visualize the learned features of neurons, we first try the method used in previous \doc{papers} on explainable deep learning~\cite{bilal2018convolutional,liu2017towards}.
% This method selects the image patches that highly activate a neuron to represent its learned feature.
% However, we discovered that when handling very deep CNNs (e.g., ResNet101~\cite{He2016_CVPR_residual}), this method cannot illustrate the \mengchen{exact} region in each image patch that highly activates a feature map neuron, especially for the neurons in top layers.
% This is because the activations of neurons in top layers of a very deep CNN are influenced by a large image patch.
% For example, the neurons in more than 10 layers are influenced by all \doc{the} pixels in an image in ResNet101.
% Thus, we employ the discrepancy map~\cite{zhou2014object} to highlight which region in the image actually highly activates a neuron and treat this region as the learned feature of this neuron.
% To calculate the discrepancy map for a neuron, Zhou et al.~\cite{zhou2014object} occluded a very small patch of an image (8 pixels$\times$ 8 pixels), and calculated the new activation of the neuron produced by the occluded image.
% If the activation changes \doc{a great deal}, the small patch is marked as important.
% This process iterates many times, and \doc{for} each iteration, a different patch is checked.
% After this process, all the important small patches of the image \doc{remain} unchanged and other pixels are deemphasized by lowering their lightness.
% For example, in Fig.~\ref{fig:neuron_vis}(a), by examining the discrepancy maps, we found that the neurons in the selected feature map learned to detect
% \kelei{a panda ear or a panda head.}
% Without detecting the important region, we may draw the wrong conclusion that the neurons learned to detect a whole panda.

\subsection{Network-level visualization}
\label{sec:vis-net}
% Next, we need to provide visual hints on this backbone to disclose the potential diverging and merging points, and further guides experts in selecting a diverging / merging point of interest (a layer in the network) to examine.
\begin{wrapfigure}{r}{0.15\textwidth}
  \begin{overpic}[width=0.9\linewidth]{fig/original-node-ratio.pdf}
    \put(15, 70){0.0}
    \put(65, 70){1.0}
  \end{overpic}
 %\vspace{-0.2in}
 \vspace{1mm} 
%  \caption{A dot plot to encode the datapath similarity in a layer group. }
\caption{Dot plot. }
 \label{fig:dot}
 \end{wrapfigure}

In our previous work~\cite{liu2018analyzing}, we employed a dot plot to visualize the difference between \textbf{two} datapaths.
% As shown in Fig.~\ref{fig:dot}, each rectangle represents a layer group, and each dot in the plot represents the activation similarity between two datapaths of a layer.
As shown in Fig.~\ref{fig:dot}, each rectangle represents a layer group, \mcrev{where layers are hierarchically grouped according to the hierarchical computation graph defined in the widely-used TensorFlow Graph Visualization~\cite{wongsuphasawat2018visualizing}.}
Each dot in the plot represents the activation similarity between two datapaths of a layer.
As a result, the dot plot is combined with the layer group to illustrate the similarities between the extracted datapaths of each layer in each layer group.
The position of a dot on the x-axis denotes the similarity value, from 0 (left) to 1 (right).
The method has been demonstrated to be useful in detecting the diverging/merging point of two datapaths (e.g., the datapaths of adversarial panda and normal panda images).
However, we have received feedback from the experts that the dot-plot-based visualization %method 
is less intuitive in revealing the overall evolution pattern of datapath merging and diverging as well as the transition between them. 
Moreover, it cannot compare three datapaths, which is specifically requested by the experts.
The experts said that in %their 
analysis, they often needed to examine the adversarial examples in the context of \jw{both} normal source examples (e.g., panda) and normal target examples (e.g., monkey) %and thus 
to identify the critical diverging/merging points. 



To tackle these issues, we \newdoc{have} develop\newdoc{ed} a river-based visual metaphor~\cite{Cui2011textflow}, which is inspired by the natural phenomenon of \newdoc{a} river merging and diverging along
\newdoc{%the
a} riverbed.
The river-based visualization has been 
\newdoc{%proved
proven} effective
\newdoc{%in
at} depicting
\newdoc{%the
}diverging and merging patterns over time~\cite{Cui2011textflow}.
As shown in Fig.~\ref{fig:case0_overview}, we use a curve to represent a datapath.
\mcrev{Considering the complexity of the current system, we do not use the curve width to encode extra information, and thus the width is always the same.}
The distance between \jw{the curves} represents the similarity between two datapaths.
The smaller the distance, the more similar the two datapaths.
\mc{\newdoc{%For the case of
When} comparing three datapaths (adversarial, normal source, and normal target examples), we employ a rule-based method to highlight \newdoc{%the
}diverging and merging patterns.
In particular, the datapath of the adversarial example stays in the middle
\newdoc{%andf
with} the other two (source and target) on
\newdoc{%each
either} side (Fig.~\ref{fig:case0_overview}).
The screen distance is proportional to the datapath distance $d_1$ (source-target).
The position of the datapath of the adversarial example is determined by
\newdoc{%keeping
retaining} the ratio of $d_2$ (adversarial - source) and $d_3$ (adversarial - target).}
% To combine this design and the backbone visualization, we embed the river-based visualization into the DAG visualization (Fig.~\ref{fig:case0_overview}). 
To better reveal how data flows in the network, we embed the river-based visualization into the DAG visualization representing the network structure (Fig.~\ref{fig:case0_overview}). 
With this combination, %datapath 
the \textbf{merging} (Fig.~\ref{fig:case0_overview} (a)), \textbf{diverging}  (Fig.~\ref{fig:case0_overview} (b)), and %the 
\textbf{transition} between \jw{datapaths} %them 
can be easily recognized by examining the distance changes. %between datapaths
(Fig.~\ref{fig:case0_overview} (c)).
For example, in Fig.~\ref{fig:case0_overview} (a), the distance between the blue curve (normal panda) and the orange curve (adversarial example)
\newdoc{%keeps on increasing
increases}.
This indicates that the critical neurons of these two datapaths are gradually
\newdoc{%less and 
becoming} less similar to each other, creating a \textbf{diverging pattern}.
While in Fig.~\ref{fig:case0_overview} (b), the distance between the orange curve (adversarial example) and the purple curve (normal monkey)
\newdoc{%keeps on decreasing
decreases}.
This indicates that the critical neurons of these two datapaths are gradually 
\newdoc{%more and
becoming} more similar to each other, creating a \textbf{merging pattern}.
Fig.~\ref{fig:case0_overview} (c) shows a transition process from the \jw{diverging} %divergence 
between a normal panda and an adversarial panda to the \jw{merging of} %merge between 
an adversarial panda and a normal monkey. 
Revealing these patterns helps experts quickly locate the layer of interest for further investigation.


\begin{figure}[bpht]
  \centering
%   \vspace{3mm}
  \begin{overpic}[width=0.95\linewidth]{fig/case-dataflow.pdf}
%   \put(7, 30){Panda}
%   \put(-1.5, 25){Adversarial}
%   \put(4, 20){Monkey}
%   \put(25.5, 25.5){$d_1$}
%   \put(30, 28){$d_2$}
%   \put(30, 23){$d_3$}
%   \put(45, 34){Diverging pattern}
%   \put(70, 30){Merging pattern}
  \end{overpic}
  \caption{
  \kelei{Visualization of three datapaths, with the illustration of (a) the diverging pattern, (b) the merging pattern, and (c) the transition from diverging to merging.}
  }
  \label{fig:case0_overview}
\end{figure}

% \noindent
% \kelei{
% \textbf{Diverging pattern.}
% For example, the orange curve in Fig.~\ref{fig:dataflow_intro}(a) obviously becomes far away from the orange curve.
% The orange curve corresponds to the adversarial example ($I_A$ in Fig.~\ref{fig:teaser-overview}(a)) and the blue curve corresponds to the original image of the adversarial example ($I_B$ in Fig.~\ref{fig:teaser-overview}(a)).
% This diverging phenomenon means the critical neurons for these two groups are no longer similar,
% which indicates the mechanisms of neurons in two adjacent layers may have a big change.
% Therefore, it helps experts locate important layers for analyzing different behaviors of the target model on visually similar examples.
% %On the other hand, the change of the purple curve is relatively slight and not useful to find reasons of misclassifications.
% }


% \noindent
% \kelei{
% \textbf{Merging pattern.}
% A typical merging pattern is displayed in Fig.~\ref{fig:dataflow_intro}(b), in which the orange curve obviously get close to the purple curve.
% The purple curve represents images that come from the misclassified class of the adversarial example ($I_C$ in Fig.~\ref{fig:teaser-overview}(a)).
% This obvious change indicates working mechanisms of neurons in two adjacent layers have a big change.
% So these two layers are meaningful for analyzing similar behaviors of the target model on visually different examples.
% }




\subsection{Layer-Level Visualization}
When examining a layer of interest, such as a layer with a diverging or merging pattern, the critical feature maps of that layer (Fig.~\ref{fig:system} (c)) are \jw{important for understanding the key features learned in that layer.} %very important to understand what key features are learned in that layer.
%The learned features 
\jw{These feature maps and corresponding learned features} are generally useful \jw{for understanding} %to understand 
why an adversarial example \jwReRe{diverges} %\newdoc{%is}diverged 
from its original category and \jwReRe{merges} %merged 
into another category.
As a result, the unique and shared feature maps between/among datapaths are expected to be encoded and visualized clearly.
To this end, we employ a treemap-based visualization to describe the set relations\newdoc{hips} among \jw{the feature maps} %different feature map set 
of different datapaths. 
The basic idea %of this formulation 
is illustrated in Fig.~\ref{fig:fm-layout-intro}.
%Fig.~\ref{fig:fm-layout-intro}
\jw{In the figure,} 
(a) shows %\jw{the Venn diagram of} 
three \jw{sets of feature maps belonging to} %feature map sets of 
three datapaths (normal panda, adversarial panda, and normal monkey), and their set relations.
We first compute the shared (intersection) and unique parts of \jw{the three sets} %different feature map sets 
(Fig.~\ref{fig:fm-layout-intro} (b)). Then a hierarchy is built based on the set inclusion relations\newdoc{hips} (Fig.~\ref{fig:fm-layout-intro} (c)). 
To have more space for displaying the shared \newdoc{%parts
}and unique part\newdoc{s} and distinguishing them clearly, we put the shared %intersection 
parts into the largest set with more feature maps.
Finally, the feature map sets and their intersection relations\newdoc{hips} are visualized with a squarified treemap layout~\cite{bruls2000squarified} (Fig.~\ref{fig:fm-layout-intro} (d)).


To better reveal the relationships 
between the shared and unique parts of different datapaths, the \jw{treemap cells of the shared parts} %shared feature map set 
are placed \jw{
\newdoc{%at
in} a %middle 
position
\newdoc{%trying to be
that is as} close \newdoc{as possible} to every} %near the 
treemap cell of %each 
related feature map sets. 
For example, the shared part, \textbf{S}, of feature map sets \textbf{A}, \textbf{B}, and \textbf{C} are placed near the centers of the three related treemap cells representing \textbf{A}, \textbf{B}, and \textbf{C} (Fig.~\ref{fig:fm-layout-intro} (d)). 
Accordingly, the treemap layout is formulated as an optimization problem 
%\jw{to minimize the distance from the center of} 
with the goal of placing the \jw{treemap cells of} shared %feature map 
sets close 
to the center of \jw{the cells of related sets:} %each related feature map sets:
\begin{equation}
\begin{aligned}
\label{eq:treemap-optimization}
% & cost = \min \sum_{S_i \in \{ 0,1\},\sum_i{S_i}\ge 2}
% (&
% f_c(\mathop{\cap}\limits_{i:S_i=1}{A_i}) - & \\
% & & \mathop{f_m}\limits_{i:S_i=1}(f_c(A_i)))^2 & 
\min \sum_{s_i \in \{ 0,1\},\sum_i{s_i}\ge 2}
(f_e(\mathop{\cap}\limits_{i:s_i=1}{A_i}) -\mathop{f_m}\limits_{i:s_i=1}(f_e(A_i)))^2,
\end{aligned}
\end{equation}
where $\mathop{\cap}\limits_{i:s_i=1}{A_i}$ is the set that contains all feature maps shared by $A_i$, for all $s_i=1$. 
$s_i$ is the status variable of $A_i$. 
$s_i=1$ indicates that $A_i$ contains the shared part $\mathop{\cap}\limits_{i:s_i=1}{A_i}$, while $s_i=0$ means that $A_i$ does not contain this set.
% $f_e(\mathop{\cap}\limits_{i:s_i=1}{A_i})$ denotes its center, while $\mathop{f_m}\limits_{i:s_i=1}(f_e(A_i))$ denotes the centroid of the centers of the feature map sets that construct such generalized intersection.
$f_e(\cdot)$ denotes the center of the treemap cell representing a set, while $\mathop{f_m}\limits_{i:s_i=1}(\cdot)$ is the mean of the centers. %of the selected feature map sets.
Accordingly, the first term represents the center of the shared feature map set $\mathop{\cap}\limits_{i:s_i=1}{A_i}$, and the second term represents the mean of the centers of the feature map sets that share $\mathop{\cap}\limits_{i:s_i=1}{A_i}$. 


This \jw{optimized} treemap-based visualization %with the aforementioned constraint 
can clearly reveal the shared and unique feature maps \jw{on} %of 
the datapaths of interest, which is useful for investigating the roles of different types of feature maps (e.g., unique or shared feature maps) in the prediction.
For example, the experts are interested in examining the unique feature maps on each datapath for a diverging point.
While for a layer with a merging pattern, the shared feature maps among datapaths are critical for the prediction analysis.

\begin{figure}[!t]
  \centering
  \vspace{4mm}
  \begin{overpic}[width=0.98\linewidth]{fig/fm-intro-layout.pdf}
  \small
  %{fig/visualization_feature-map-layout-intro.PNG}
  \put(20, 88){\textsf{(a)}}
  \put(70, 88){\textsf{(b)}}
  %\put(55, 95){\tiny $\twosi{\twosi{A}{B}}{C} = \{1,2,3\}$}
  %\put(55, 90){\tiny $(\twosi{A}{B})^\prime = \twosi{A}{B} - \mathrm{C} = \{4\}$}
  %\put(55, 85){$(\twosi{B}{C})^\prime = \twosi{B}{C} - \mathrm{A} = \{5,6\}$}
  \put(20, -2){\textsf{(d)}}
  \put(70, -2){\textsf{(c)}}
  \end{overpic}
  %\vspace{-2mm}
%   \vspace{2mm}
  \caption{
  Illustration on how to create a feature map visualization for three datapaths. %at a layer of interest. 
(a) The three sets of feature maps %sets of the datapaths 
at a selected layer;
(b) The intersection relations\newdoc{hips} among the sets;
(c) %Build a tree 
A hierarchy based on the set inclusion relations\newdoc{hips};
(d) The treemap-based visualization of feature maps. 
%The shade of green encodes the activation or activation difference between two datapaths. %The darker green indicates a higher value. 
}
\label{fig:fm-layout-intro}
\end{figure}

To facilitate the identification of salient feature maps, two types of encoding are employed for activation and contribution, respectively.

\noindent\textbf{Encoding the activation difference}.
We select the maximum neuron activation in a feature map to represent its activation, with
\newdoc{%an aim to emphasize
the aim of emphasizing} the most salient feature detected by the feature map.
The solid filling style $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_solid.pdf}}}$ is used to encode the activation difference between two datapaths.
Taking datapaths \textbf{A} and \textbf{B}
\newdoc{%for
as an} example, their activation difference is
\textit{acti}(\textbf{A})-\textit{acti}(\textbf{B}). 
% When encoding the the activation of the feature map, the higher filling height indicates that the learned features are more salient. 
% When encoding the activation difference between two datapaths (e.g., \textit{activation}(\textbf{A})-\textit{activation}(\textbf{B})), 
The larger \newdoc{the} value, the higher \newdoc{the} filling, %height 
\jw{which} indicates that the learned feature \jw{is more salient in \textbf{A} than in \textbf{B}.} %are the more salient feature in \textbf{A} instead of \textbf{B}.


\noindent\textbf{Encoding the contribution}.
%If the expert selects part of neurons in a specific feature map (focused feature map), s/he also wants to know how the neurons corresponding the selected feature map area at previous layers contribute to the activation of the selected neurons.
\jw{A subset of neurons in a specific feature map can be selected as an area of interest \todo{(Fig.~\ref{fig:teaser-overview}D)}. Experts can trace how corresponding neurons in previous layers contribute to the activations of the selected neurons.} 
This is useful for identifying the key %learned 
\newdoc{%features learned
learned features} that lead to
\newdoc{%the
}diverging or merging \jw{of datapaths}. 
In addition, to facilitate the analysis of the diverging/merging patterns for adversarial examples, it is essential to understand how feature maps at each layer contribute to the final prediction. 
In our visualization, the dotted filling style $\vcenter{\hbox{\includegraphics[height=1.5\fontcharht\font`\B]{fig/glyph_dotted.pdf}}}$ is employed to encode 
% the contribution of a feature map (or the selected region of a feature map) to the final prediction (or the neuron activation of the selected region in the focused feature map).
the contribution from corresponding neurons in previous \jw{layers} %feature maps 
to the activation of the neurons in the focused area or to the final prediction.
The higher filling %height 
represents a larger contribution value. 



\subsection{Contribution Analysis}
% \todo{rewriting} 
% \noindent \textbf{Contribution analysis.}
When
\newdoc{%the
an} expert finds a pattern of interest (e.g., a \todo{critical feature map} in a diverging point or merging point), s/he often \jw{wants} %needs 
to analyze the major cause that 
leads %\newdoc{%leadsled} 
to the pattern.
To this end, we \newdoc{have} develop\newdoc{ed} a contribution analysis method to compute the contribution of the previous feature maps to the neuron activation of the feature map of interest (target feature map).

Initially, the contribution analysis is performed based on the whole target feature map.
We formulate this problem as a subset selection problem.
It aims to select a minimum number of feature maps that can maximally preserve the activation of the target feature map.  
This formulation is similar to the datapath extraction discussed in Sec.~\ref{sec:datapath}.
As a result, we also employ the continuous optimization method to select the feature maps and compute the corresponding contribution.
In particular, we replace the first term in Eq.~(\ref{eq:dp-ext-new-3}) with the preservation of the activation of the target feature map:
\begin{equation}
\begin{aligned}
\label{eq:vis-contribution-analysis}
\vecz{opt}^i = & \underset{\vecz{prev}^i\in [0,1]^{n}}{\mathop{\arg \min }} (f(x^i)-f(x^i;\vecz{prev}^i))^2 \\
& + \lambda |\vecz{prev}^i|+ \gamma \sum_{j \in [1, m], j \neq i}||\vecz{prev}^j - \vecz{prev}^i||_2,
\end{aligned}
\end{equation}
where $f(x^i)$ is the %selected 
neuron activation of the target feature map on example $x^i$ and $f(x^i;\vecz{prev}^j)$
%is according neuron activation with consideration of
\keleiReRe{is the corresponding neuron activation
\newdoc{%with
in} consideration of}
the previous feature map contributions $\vecz{prev}^j$.
\todo{$m$ is the number of datapaths being analyzed.}
%the neuron activation of the target feature map on example $x$,
%\jw{if we only consider the feature map subset $\vecz{}^j$}. 
% the neuron subset represented by $\vecz{s}$ of each selected feature map.
This optimization problem can be solved similarly with our proposed algorithm in Sec.~\ref{sec:datapath}.





% When an expert find an interested feature map based on the extracted datapaths,
% he/she then inspects the previous layers to examine the more specific reason that affects this feature map.
% Therefore, it is useful for experts to identify feature maps that have main contribution to the selected feature map.
%We formulate this problem as a subset selection problem and solve it similarly with our proposed algorithm in Sec.~\ref{sec:datapath}:
%By replacing the first term in Eq.~\ref{eq:dp-ext-new-3} with the change of the selected feature map,
%the final solution is contribution that each optimized feature map make to the selected feature map.
% \kelei{
% We formulate this problem as a subset selection problem, replace the first term in Eq.~\ref{eq:dp-ext-new-3} with the change of the selected feature map:
% \begin{equation}
% \begin{aligned}
% \label{eq:vis-contribution-analysis}
% \vecz{opt} = \underset{\vecz{s}\in [0,1]^n}{\mathop{\arg \min }} & (f(x)-f(x;\vecz{s}))^2 \\
% & + \lambda |\vecz{s}|+ \gamma \sum_{j \in [1, i-1]}||\vecz{s} - \vecz{c}||_2,
% \end{aligned}
% \end{equation}
% Where $f(x)$ is the activation of the selected feature map on example $x$,
% and $f(x;\vecz{s})$ is the activation on example $x$ if we only consider the neuron subset represented by $\vecz{s}$.
% This problem can be solved similarly with our proposed algorithm in Sec.~\ref{sec:datapath}.
% }

When using this contribution analysis method to analyze the adversarial noise, we
\newdoc{%find
discover} an issue. 
As shown in Fig.~\ref{fig:vis-focus-contribution} (a), if all the neurons of the target feature map are considered, some irrelevant feature maps, such as FM1 and FM2, are ranked highest, while the relevant one, FM3, is ranked
\newdoc{%as the
}third. %one. 
This is because, in addition to 
the feature that is misled by the adversarial noise, other irrelevant features with high neuron activation, are also considered. 
These irrelevant features may trigger several irrelevant feature maps and rank them higher.

To tackle this issue, we allow
\newdoc{%the
}expert\newdoc{s} to only select neurons (Fig.\ref{fig:vis-focus-contribution}A) that are highly activated on the adversarial noise and examine the influence of other feature maps
\newdoc{%to
on} these selected neurons.
For example, when an expert examines a feature map of interest (e.g., Fig.~\ref{fig:teaser-overview}C),
\keleiRe{
%\sout{he}
s/he} finds that a certain area of the example is identified as a panda's ear.
S/he then checks the previous layers to investigate the
\newdoc{%cause
reason} why this area
is activated by the neurons.
Therefore, it is useful for the expert to focus on the neurons in this area and check the contribution of the previous feature maps to these selected neurons in the prediction.
The key challenge of this problem is to calculate the contribution of the corresponding neurons in each of the previous feature maps. 
Here the corresponding neurons correspond to the selected neurons in the target feature map.
Similarly, we also aim to select a minimum number of feature maps that can maximally preserve the activation of the selected neurons in the target feature map.  
% It can be formulated as a subset selection problem.
Accordingly, we change the optimization variable $z_s$ in Eq.~(\ref{eq:vis-contribution-analysis}) from the whole feature map to the corresponding neurons:
% \begin{equation}
% \label{eq:vis-partial-analysis-fm}
% \begin{aligned}
% \vecz{opt,p}^i = & \underset{\vecz{prev,p}^i\in [0,1]^{n}}{\mathop{\arg \min }} (f(x^i)-f(x^i;\vecz{prev,p}^i))^2 + \lambda |\vecz{prev,p}^i|\\
% & + \gamma \sum_{j \in [1, m], j \neq i}||\vecz{prev,p}^j - \vecz{prev,p}^i||_2,
% \end{aligned}
% \end{equation}

\begin{align} 
\label{eq:vis-partial-analysis-fm}
\vecz{opt,p}^i = & \underset{\vecz{prev,p}^i\in [0,1]^{n}}{\mathop{\arg \min }} (f(x^i)-f(x^i;\vecz{prev,p}^i))^2 + \lambda |\vecz{prev,p}^i|\notag\\
& + \gamma \sum_{j \in [1, m], j \neq i}||\vecz{prev,p}^j - \vecz{prev,p}^i||_2,
\end{align} 
where $\vecz{prev,p}=[z^1_{prev,p}, \cdots , z^n_{prev,p}]$.
% $z_{prev,p}^k \in [0,1]$ approximates the contribution of the neurons in the focused area of $k$-th feature map to the final prediction.
$z_{prev,p}^k \in [0,1]$ approximates the contribution of the neurons in the focused area of $k$-th feature map to the activation of the selected neurons in the target feature map.
% We similarly solve it with our proposed algorithm in Sec.~\ref{sec:datapath}.

The top 3 most contributed feature maps identified by the new method are shown in (Fig.\ref{fig:vis-focus-contribution} (b), where the most relevant one, FM3, ranks first.

% \noindent \textbf{Time complexity.} \mcrev{The contribution analysis is the only part that cannot be pre-computed (the offline pre-computation usually takes a few minutes) because the contribution is calculated based on the selected neurons.
% It usually takes about $5$ seconds to calculate 
% \newdoc{%such
% the} contribution using SGD to solve Eq.~(\ref{eq:vis-partial-analysis-fm}).
% \newdoc{%For acceleration
% To accelerate the process}, we can use the quadratic approximation
% \newdoc{%in
% from} our previous work~\cite{liu2018analyzing}, which
% \newdoc{%has better time efficiency
% is faster} (computation time $<1s$) but
% \newdoc{%worse analysis accuracy.
% less accurate.}
% \newdoc{%As
% Since} our target users (machine learning experts) focus more on analysis accuracy, the SGD-based solution is set as default.
% \newdoc{%The users
% Users} can switch to the approximated contribution analysis in the interface.
% }


\begin{figure}[thbp]
  \centering
  \begin{overpic}[width=0.98\linewidth]{fig/focus-and-contribution.pdf}
  \small
  \end{overpic}
  \caption{The top 3 most contributed feature maps identified by considering a) the whole feature map of interest; b) part of the feature map of interest.}
  \label{fig:vis-focus-contribution}
  \vspace{-5mm}
\end{figure}

% \noindent \textbf{Local analysis.}
% \kelei{
% When an expert inspects an interested feature map (e.g., Fig.~\ref{fig:neuron_vis}),
% he finds a certain area of the example that is identified as a panda's ear.
% He then inspects the previous layers to examine the cause why this area is activated by the neurons.
% Therefore, it is useful for experts to focus on the neurons in this area and mask out the influence of other neurons during the following analysis.
% The key challenge of this problem is to calculate the importance of the focused area in each feature map. 
% It can be formulated as a subset selection problem.
% We change the optimization variable in Eq.~\ref{eq:dp-ext-new-3} from the importance of each feature map to the importance of the neurons in the focused area:
% \begin{equation}
% \label{eq:vis-partial-analysis-fm}
% \begin{aligned}
% \vecz{opt,p} = \underset{\vecz{s,p}\in [0,1]^n}{\mathop{\arg \min }}\, & (f(x)-f(x;\vecz{s,p}))^2 + \lambda |\vecz{s,p}| \\
% & + \gamma \sum_{j \in [1, i-1]}||\vecz{s,p} - \vecz{c,p}||_2.
% \end{aligned}
% \end{equation}
% where $\vecz{s,p}=[z^1_{s,p}, \cdots , z^n_{s,p}]$.
% $z_{s,p}^j \in [0,1]$ approximates the contribution of the neurons in the focused area of $j$-th feature map to the final prediction.
% We similarly solve it with our proposed algorithm in Sec.~\ref{sec:datapath}.
% }



% \begin{figure}[htbp]
%   \centering
%   \vspace{-2mm}
%   \includegraphics[width=\linewidth]{fig/layer_vis.pdf}
%   \caption{Comparison between DAG visualization and our segmented DAG visualization: (a) DAG visualization showing 49 layers of ResNet101 simultaneously; (b)  showing the same layers with our segmented DAG visualization; (c) the segmentation result calculated by only considering the empty space at the end of each segment.
%   }
%   \label{fig:layer_vis}
% \end{figure}

% \kelei{
% \subsection{Flow Visualization}
% Since experts have more interests on layers that have obvious change on relations among datapaths,
% it is useful to provide an overview of how datapaths diverge and merge (\textbf{R2}).
% However, the original visual hint (dot plot) is not good at displaying relations when there are more than two groups.
% Triggered by TextFlow~\cite{Wang2016_VAST}, we extend the DAG layout to a data flow visualization with embedded threads (Fig.~\ref{fig:teaser-overview} (b)).
% For example, Fig.~\ref{fig:case0_examineUnit23} (a) is a part of the layer-level visualization with Fig.~\ref{fig:case0_examineUnit3} (a) as input example groups.
% Data flow is employed to connect layers and represent the direction that data flows through layers in a model.
% Each embedded thread inside the data flow represents an example group.
% As experts focus on analyzing adversarial examples, the corresponding thread is always located at the middle of data flow as baseline.
% The similarities between adversarial examples and other groups are encoded as the distance between corresponding threads.
% }


% \noindent \textbf{\normalsize Layout.}
% At the layer level, we focus on illustrating how layers are connected.
% A widely-used approach is to formulate a CNN as a DAG (directed acyclic graph), where each layer is a node and their connections are edges~\cite{kahng2018acti,liu2018analyzing,wongsuphasawat2018visualizing}.
% Based on this formulation, a node-link diagram is employed to visualize the layers and their connections.
% To handle large CNNs, a hierarchy of the layers can be built, where each leaf node is a layer and each non-leaf node is a layer group~\cite{wongsuphasawat2018visualizing}.
% Then the top level of this layer hierarchy is shown by default and experts are able to expand the layer group of interest to examine child layers or layer groups.
% This design is suitable for CNNs with relatively shallow depth, such as the VGG net~\cite{simonyan2014very}, \doc{which has} 15-20 layers.
% However, for state-of-the-art CNNs, such as ResNet with 50-200 layers~\cite{He2016_CVPR_residual}, when experts zoom in to the lower levels of this hierarchy (e.g., the individual layers of the layer group ``block4'' in ResNet101), the visualization suffers from a long skinny strip with a very high aspect ratio (Fig.~\ref{fig:layer_vis} (a)), which is hard to explore and analyze.

% To solve this problem, we develop a segmented DAG visualization, which contains the following two steps. 

% \textit{Tree cut.} 
% We first use a treecut algorithm~\cite{cui2014hierarchical} to select an initial set of layers (around 50 layers). 
% In this algorithm, the DOI measures the datapath difference between two sets of images (e.g., adversarial examples and normal examples).
% Then the DAG layout algorithm in~\cite{wongsuphasawat2018visualizing} is employed to calculate the position of each layer.

% \textit{Segmentation.}
% Triggered by the segmented timeline~\cite{brehmer2017timelines}, we propose \doc{segmenting} the initial DAG into several parts, and \doc{visualizing} the segmented parts from top to bottom.
% As shown in Fig.~\ref{fig:layer_vis} (b), our segmented DAG visualization effectively illustrates the connections among dozens of layers with good aspect ratios.  
% The key challenge of segmenting a DAG is to decide where to segment \doc{it}.
% We formulate the segmentation problem as a ``printing neatly'' problem~\cite{cormen2009introduction}, \doc{in which} we aim to minimize the cost function that sums up the empty space at the end of each line while ensuring that no word is \doc{off} screen.
% This optimization method is suitable for a CNN with a chain structure, such as VGG net~\cite{simonyan2014very}.
% However, state-of-the-art CNNs (e.g., ResNet~\cite{He2016_CVPR_residual}, and DenseNet~\cite{huang2017densely}) often contain basic building blocks, whose layers can split and merge (e.g., Fig.~\ref{fig:layer_vis}A).
% These building blocks are often connected with others as a chain.
% Directly minimizing the above cost function may cut the basic building blocks apart, which hinders the understanding of the network structure.
% To solve this problem, we add a regularization term to the cost function to penalize a segmentation scheme that cuts a building block into two parts:
% \begin{equation}
% \label{eq:segment}
% \underset{e_i \geq 0}{\mathop{\min }}\, \sum\limits_{i=1}^{k-1}{e_i + \lambda c_i},
% \end{equation}
% where $k$ is the number of segments, $e_i$ is the empty space at the end of segment $i$, $c_i$ represents whether a building block is cut by segment  $i$, and $\lambda$ is used to balance the two terms.
% In AEVis, experts can interactively modify $\lambda$.
% Eq.~(\ref{eq:segment}) can be efficiently solved using dynamic programming.
% As shown in Fig.~\ref{fig:layer_vis}, if we only consider the empty-space objective, \doc{building block A} will be cut into two parts (Fig.~\ref{fig:layer_vis} (c)).
% Adding the regularization term can avoid unnecessary cuts by balancing between the small empty space and the protection of the building blocks (Fig.~\ref{fig:layer_vis} (b)).

% \noindent \textbf{\normalsize Visual hint.}
% Showing how the layers are connected is not enough in guiding experts to find the layer of interest.
% Thus, for each node (a layer or layer group) in the segmented DAG, we provide a visual statistical description of the datapath(s) in that layer (group).
% Because there is limited space for each node and a layer group usually contains dozens of layers, we employ a dot plot as the visual hint, which is a compact visualization and 

% widely used for relatively small datasets~\cite{rodrigues2018nonlinear}.
% In particular, in a dot plot, each dot represents a layer (Fig.~\ref{fig:dot}).
% The position of a dot on the x-axis denotes a high-level statistics of the datapath(s) in that layer (Fig.~\ref{fig:dot}),
% such as the activation similarity between two datapaths (the datapath for adversarial examples and the one for normal examples).
% Examining the dot plots node by node helps experts detect the ``diverging point,'' where a normal image and its corresponding adversarial example diverge into different predictions (Fig.~\ref{fig:case0_overview}). 


% \subsection{Feature-map-level Visualization}
% When an expert detects a layer of interest, he/she then zooms in to the layer to examine the critical feature maps in that layer.
% To preserve the analysis context, we visualize the feature maps in the selected layer as \doc{the} focus and other layers are shown as context. (Fig.~\ref{fig:teaser} (b)).

% \noindent \textbf{\normalsize Layout.}
% The belonging relationships between the feature maps and the extracted datapaths in one layer, including the unique feature maps of each datapath and the shared ones between/among them, are very useful for understanding the roles of these feature maps. 
% To illustrate such relationships, we design two alternative visualizations.
% In the first design (Fig.~\ref{fig:fm_vis} (a)), we use a pie-chart-based glyph to show the relationship between a feature map and the datapaths (Fig.~\ref{fig:fm_vis}A).
% In particular, the feature maps of different datapaths are encoded \doc{with} different colors and the one shared by multiple datapaths are represented by a pie chart.
% In the second design, we employ a treemap to illustrate the overlapping relationships between the datapaths.
% For example, feature map B in Fig.~\ref{fig:fm_vis} (b) is a shared feature map of the two datapaths, while feature map C is a unique feature map for the blue datapath.
% This design is triggered by the Euler diagram~\cite{alsallakh2014visualizing}, \doc{in which} sets are represented by closed curves (e.g. rectangles) and the relationships among sets are illustrated by the curve overlaps.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.85\linewidth]{fig/fm_vis.pdf}
%   \vspace{-2mm}
%   \caption{Two alternative designs of feature-map-level visualization: (a) a pie chart is utilized to encode the belonging datapaths of a feature map; (b) a treemap is employed to encode the relationships among datapaths.}
%   \label{fig:fm_vis}
%   \vspace{-4mm}
% \end{figure}

% After we presented these two designs to the experts, the experts commented that they were both acceptable, but they preferred the second one \doc{since} they are very familiar with the Euler-diagram-based design.
% The experts further commented that they often used Euler diagrams to understand the set relationships in their analysis tasks. 
% In addition, the size of each part is clearly conveyed in this design, which is a very important factor in their analysis. 
% Thus, we adopt the second design in AEVis.
% To reduce the visual clutter caused by a large number of feature maps, we use K-Means~\cite{christopher2006_PRML} to cluster the feature maps by their activations.
% Based on the clustering results, we arrange the feature map clusters on a grid in a treemap cell. 
% Experts can expand a feature map cluster of interest and examine the corresponding feature maps.

% \begin{wrapfigure}{r}{0.15\textwidth}
% \vspace{-0.2in}
% \includegraphics[width=0.15\textwidth]{fig/fm_vis_hint.pdf}
% \vspace{-0.2in}
% \caption{The visual hints for a feature map cluster. FM is short for feature map.}
% \label{fig:fm_vis_hint}
% \end{wrapfigure}

% \noindent \textbf{\normalsize Visual hint.}
% Although the treemap-based design reveals the shared/unique feature maps very well, it  \doc{does not significantly help} to efficiently select an individual feature map cluster of interest for further examination.
% To this end, for each cluster, we illustrate its average importance ($z_j^i$ in Eq.~(\ref{eq:dp-cont}), Sec.~\ref{sec:datapath}) or average activation, because experts usually start their analysis from the most critical or most highly activated feature maps. 
% The averaged importance/activation of a feature map cluster is encoded by the color of the feature map cluster (Fig.~\ref{fig:fm_vis_hint}).
% In addition to importance/activation, we also encode the size of a feature map cluster because it is a basic information for a cluster.
% We employ a series of stacked rectangles to represent a feature map cluster (Fig.~\ref{fig:fm_vis_hint}).
% Triggered by Squares~\cite{ren2017squares}, we employ the number of stacked rectangles to encode the size of a cluster, which is proportional to the log of the cluster size. 
% For \doc{the sake of} consistency, a cluster with only one feature map in it is shown as a single rectangle.\looseness=-1


% \subsection{Neuron-level Visualization}
% When an expert finds a feature map of interest, AEVis allows him/her to examine the neurons in that feature map.
% As there are hundreds or even thousands of neurons in a feature map and dozens of images are often analyzed simultaneously, we cannot show all the activations in place due to the limited space.
% Thus, we add a neuron panel (Fig.~\ref{fig:teaser}) to show the neurons.
% To preserve the visual link~\cite{Steinberger2011TVCG_link} of the selected feature map and the corresponding neurons, we add the same label to the feature map and the neurons (Fig.~\ref{fig:neuron_vis}A).  

% \noindent \textbf{\normalsize Layout.}
% In a feature map, the neurons are naturally organized on a grid.
% \mengchen{The position of a neuron is determined by the position of the image patch that influences the activation of this neuron~\cite{goodfellow2016deep}.}

% \noindent \textbf{\normalsize Visual hint.}
% Following previous research~\cite{bilal2018convolutional,liu2017towards},  we employ the learned features of neurons and the activations of the neurons to help expert understand the roles of the neurons for the prediction.

% The activation of a neuron is represented by its color (red: negative activation; green: positive activation).
% Combining the color coding and the grid-based layout of neurons, experts can detect which part of the image highly activates the neurons in the feature map.
% For example, in Fig.~\ref{fig:neuron_vis}, we can find the neurons on the top right corner are highly activated, which corresponds to the panda head in the image.

% To visualize the learned features of neurons, we first try the method used in previous \doc{papers} on explainable deep learning~\cite{bilal2018convolutional,liu2017towards}.
% This method selects the image patches that highly activate a neuron to represent its learned feature.
% However, we discovered that when handling very deep CNNs (e.g., ResNet101~\cite{He2016_CVPR_residual}), this method cannot illustrate the \mengchen{exact} region in each image patch that highly activates a feature map neuron, especially for the neurons in top layers.
% \doc{This is because} the activations of neurons in top layers of a very deep CNN are influenced by a large image patch.
% For example, the neurons in more than \mengchen{10 layers} are influenced by all \doc{the} pixels in an image in ResNet101.
% Thus, we employ the discrepancy map~\cite{zhou2014object} to highlight which region in the image actually highly activates a neuron and treat this region as the learned feature of this neuron.
% To calculate the discrepancy map for a neuron, Zhou et al.~\cite{zhou2014object} occluded a very small patch of an image (8 pixels$\times$ 8 pixels), and calculated the new activation of the neuron produced by the occluded image.
% If the activation changes \doc{a great deal}, the small patch is marked as important.
% This process iterates many times, and \doc{for} each iteration, a different patch is checked.
% After this process, all the important small patches of the image \doc{remain} unchanged and other pixels are deemphasized by lowering their lightness.
% For example, in Fig.~\ref{fig:neuron_vis}, by examining the discrepancy maps, we \doc{found} that the neurons in the selected feature map learn\doc{ed} to detect a panda head.
% Without detecting the important region, we may draw \doc{the} wrong conclusion that the neurons learn\doc{ed} to detect a whole panda. 

% \begin{figure}[htbp]
%   \centering
%   \vspace{-1mm}
%   \includegraphics[width=0.7\linewidth]{fig/neuron_vis.pdf}
%   \vspace{-2mm}
%   \caption{Neuron-level visualization: (a) the learned feature is shown as discrepancy maps; (b) activations are shown as a heat map.}
%   \vspace{-2mm}
%   \label{fig:neuron_vis}
% \end{figure}


==> background.tex <==
\section{Background}\label{sec:back}

In this section, we introduce how to generate adversarial examples.
